Scalable Benchmarking and Robust Learning for Noise-Free Ego-Motion and 3D Reconstruction from Noisy Video

We aim to redefine robust ego-motion estimation and photorealistic 3D reconstruction by addressing a critical limitation: the reliance on noise-free data in existing models. While such sanitized conditions simplify evaluation, they fail to capture the unpredictable, noisy complexities of real-world environments. Dynamic motion, sensor imperfections, and synchronization perturbations lead to sharp performance declines when these models are deployed in practice, revealing an urgent need for frameworks that embrace and excel under real-world noise. To bridge this gap, we tackle three core challenges: scalable data generation, comprehensive benchmarking, and model robustness enhancement. First, we introduce a scalable noisy data synthesis pipeline that generates diverse datasets simulating complex motion, sensor imperfections, and synchronization errors. Second, we leverage this pipeline to create Robust-Ego3D, a benchmark rigorously designed to expose noise-induced performance degradation, highlighting the limitations of current learning-based methods in ego-motion accuracy and 3D reconstruction quality. Third, we propose Correspondence-guided Gaussian Splatting (CorrGS), a novel test-time adaptation method that progressively refines an internal clean 3D representation by aligning noisy observations with rendered RGB-D frames from clean 3D map, enhancing geometric alignment and appearance restoration through visual correspondence. Extensive experiments on synthetic and real-world data demonstrate that CorrGS consistently outperforms prior state-of-the-art methods, particularly in scenarios involving rapid motion and dynamic illumination.

==> figs/fig_case_study_stereo_slam_euroc_baseline_perturb.tex <==
\begin{figure*}[t]
	\centering
\includegraphics[width=\textwidth]{figures/case_study_stereo_slam_euroc_baseline_perturb.pdf} 
	\caption{\textbf{Effect of perturbations on the stereo camera baseline and inter-camera transformation matrix in a stereo SLAM system.} We introduce random noise $\eta$ along the axis of the stereo camera baseline length. The noise is sampled from a Gaussian distribution with zero mean and variance $\sigma^2$, represented as $\eta \sim \mathcal{N}(0, \sigma^2)$. We illustrate (\textbf{a}) the clean setting without noise and two perturbed settings with two severity levels of noise: (\textbf{b}) $\sigma=0.001$ [m] and (\textbf{c}) $\sigma=0.01$ [m] (with three runs each). For this analysis, we provide a qualitative comparison using the EuRoC~\cite{Burri25012016} dataset. The predefined camera baseline length is set to 0.1 meters, and the stereo camera input setting of the ORBSLAM3~\cite{orbslam3} model is employed. Additionally, we include quantitative metrics to quatify trajectory estimation error, \textit{i.e.}, 'Trans', 'Scale', and 'TransGT', with all values expressed in centimeters. For more details about these metrics, please refer to the ORBSLAM3~\cite{orbslam3} literature.} 
	\label{fig:stereo-slam-baseline-perturb}
\end{figure*}

==> figs/fig_correlation_between_slam_models.tex <==
\begin{figure}[t]
	\centering
\includegraphics[width=0.44\textwidth]{figures/spearman_correlation_perturbation_plot_method_static.pdf} % \hfill 
\includegraphics[width=0.44\textwidth]{figures/spearman_correlation_perturbation_plot_method.pdf} 

	\caption{\textbf{Correlation of perturbed performance (ATE) across different multi-modal (RGB-D) SLAM models} under static (\textbf{Left}) and dynamic (\textbf{Right}) image perturbation. The pair-wise correlation strength is quantified via Spearman’s rank correlation coefficient~\citep{spearman1961proof}.}%\vspace{-2mm}
	\label{fig:correlation_perturbed_image_ate-method}
\end{figure}


==> figs/fig_depth_perturbation.tex <==
\begin{figure}[t!]
	\centering
\includegraphics[width=0.48\textwidth]{figures/depth-perturbation.pdf} 
	\caption{\textbf{Taxonomy of sensor-level perturbations for depth imaging}. We introduce four perturbations to mimic the perception noises (\textit{i.e.}, random noises and missing) and the limited perception field of depth sensors.
}
	\label{fig:depth-corruption}
\end{figure}

==> figs/fig_orbslam3_result_all.tex <==
\begin{figure*}[t]
	\centering
\includegraphics[width=\textwidth]{figures/neural-slam-all-0529.pdf}
	\caption{\xxh{Performance (measured by ATE$\downarrow$ (m)) of Neural SLAM models  under diverse perturbations. For visualization, sequences resulting in failure are assigned an ATE value of 1.0.}}
	\label{fig:neural-all}
\end{figure*}

\begin{figure*}[t]
	\centering
\includegraphics[width=\textwidth]{figures/ORB-Result-ALL-New-0529.pdf}
	\caption{\xxh{Performance (measured by ATE$\downarrow$ (m), RPE$\downarrow$ (m), and SR$\uparrow$) of ORB-SLAM3~\cite{orbslam3}. Sequences resulting in failure are assigned an ATE/RPE value of 1.0 and a Success Rate of 0. }}\vspace{-2mm}
	\label{fig:ORBSLAM-all}
\end{figure*}

==> figs/fig_orbslam_analysis_gaussian_blur.tex <==
\begin{figure}[h!]
	\centering
\vspace{-2mm}
\includegraphics[width=0.48\textwidth]{figures/orbslam_analysis_gaussian_blur.pdf} 
	\caption{{Effect of \textit{Gaussian Blur} RGB imaging perturbation (\textbf{Top}) on the quality of detected ORB features} (\textbf{Bottom}), which are marked as green dots, for ORB-SLAM3~\citep{orbslam3}. }%\vspace{-2mm}
	\label{fig:orbslam-gaussian-blur} % \textcolor{blue}
 	\centering
\vspace{3mm}
\includegraphics[width=0.23\textwidth]{figures/ape_kps_analysis.pdf} 
\includegraphics[width=0.23\textwidth]{figures/ape_mps_analysis.pdf} 
	\caption{{Correlation between trajectory estimation accuracy} {and the average number of detected} (\textbf{Left}) {and tracked} (\textbf{Right}) {ORB features for ORB-SLAM3}~\citep{orbslam3} model (RGB-D setting) under different severity level of Gaussian Blur image-level perturbation. Pearson correlation coefficient~\citep{cohen2009pearson} is reported. }%\vspace{-7mm}
	\label{fig:correlation-orb-accuracy}
\end{figure}

==> figs/fig_perturbation_taxonomy_for_SLAM.tex <==
\begin{figure}[t!]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/perturbation_taxonomy.pdf} 
	\caption{\textbf{Taxonomy of perturbations for SLAM.} Given (\textbf{a}) the original (clean) sensor stream and (\textbf{b}) trajectory, our noisy data synthesis pipeline enables the simulation of (\textbf{c}) sensor corruption (for both RGB images and depth maps), (\textbf{d}) trajectory perturbations, and (\textbf{e}) multi-sensor misalignment for the multi-modal input setting.\textcolor{red}{remake this figure to illustrate the relationship between different perturbations and their order in the synthesis procedure}}
	\label{fig:all-perturb-taxonomy}
\end{figure}

==> figs/fig_qualitative_result_trajectory_perturbation.tex <==
\begin{figure*}[t!]
	\centering
	\includegraphics[width=\textwidth]{figures/traj-ptb-qualitative_all.pdf} 
	\caption{\textbf{Illustration of trajectory deviations under different severity levels, the faster motion effect, and the multi-sensor misalignment effect.} We also show qualitative results of an advanced real-time SLAM model, \textit{i.e.}, CO-SLAM~\cite{coslam}. The impact of translation deviation, rotation deviation, {faster motion}, and sensor misalignment perturbations is assessed. For clarity, we visualize the projected trajectory on the horizontal x-y plane derived from the 3D trajectory, which shows that slight trajectory deviations can have a  significant impact on the trajectory estimation performance, measured by ATE.}%\vspace{-2mm}
	\label{fig:taxonomy-trajectory-misalign-perturbation}
\end{figure*} % , which induces small observation change in the neighboring frames (as is shown in the Fig.~\ref{fig:trajectory-perturbation-illustration}),



==> figs/fig_result_fast_motion.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/qualitative_result_coslam_faster_motion.png} 
	\caption{Effect of \textit{Faster Motion} perturbation on the performance for each scene in the Replica Dataset. We visualize the 3D point cloud reconstruction of an environment, accompanied by graphs comparing predicted trajectory (in blue) with ground truth trajectory (in black).}%\vspace{-2mm}
	\label{fig:faster-motion-coslam-qualitative}
\end{figure}

==> figs/fig_simulator_pipeline_bak.tex <==
\begin{figure*}[ht]
	\centering	\includegraphics[width=0.8\textwidth]{figures/RobuSLAM_Simulation_Pipeline.pdf} 
	\caption{\textbf{Robust-SLAM Simulation Pipeline Overview.} (a) Data Synthesis: Modular, robot-centric framework couples robot dynamics with advanced physics and sensor configurations for accurate 3D scene-derived sensor streams. (b) Perturbation: Dual-layered composers introduce variability in trajectory and sensor data. (c) SLAM Evaluation: Synthesized and perturbed data facilitates rigorous SLAM benchmarking. }%\vspace{-2mm}
	\label{fig:pipeline}
\end{figure*}

==> figs/fig_stereo_slam_perturb.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results-stereo/MH01_stereo.pdf}
        \caption{No noise; \textit{MH01} sequence.}
        \label{fig:minipage1}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results-stereo/MH02_stereo.pdf}
        \caption{No noise; \textit{MH02} sequence.}
        \label{fig:minipage2}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results-stereo/MH03_stereo.pdf}
        \caption{No noise; \textit{MH03} sequence.}
        \label{fig:minipage3}
    \end{minipage}

    \vspace{0.2cm}

    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results-stereo/MH01_stereo_0dot001.pdf}
        \caption{$\eta \sim \mathcal{N}(0, 0.001)$; \textit{MH01} sequence.}
        \label{fig:minipage4}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results-stereo/MH02_stereo_0dot001.pdf}
        \caption{$\eta \sim \mathcal{N}(0, 0.001)$; \textit{MH02} sequence.}
        \label{fig:minipage5}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results-stereo/MH03_stereo_0dot001.pdf}
        \caption{$\eta \sim \mathcal{N}(0, 0.001)$; \textit{MH03} sequence.}
        \label{fig:minipage6}
    \end{minipage}

    \vspace{0.2cm}

    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results/MH01_stereo_0dot01.pdf}
        \caption{$\eta \sim \mathcal{N}(0, 0.01)$; \textit{MH01} sequence.}
        \label{fig:minipage7}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results-stereo/MH02_stereo_0dot01.pdf}
        \caption{$\eta \sim \mathcal{N}(0, 0.01)$; \textit{MH02} sequence.}
        \label{fig:minipage8}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results/MH03_stereo_0dot01.pdf}
        \caption{$\eta \sim \mathcal{N}(0, 0.01)$; \textit{MH03} sequence.}
        \label{fig:minipage9}
    \end{minipage}

    \caption{\textbf{Effect of perturbations on the stereo camera baseline for the ORBSLAM3~\citep{orbslam3} SLAM model with the stereo input setting.} We introduce a random noise $\eta$ along the axis of the stereo camera baseline. The noise is sampled from a Gaussian distribution with zero mean and variance $\sigma^2$, represented as $\eta \sim \mathcal{N}(0, \sigma^2)$. Here, we show the qualitative comparisons on three sequences of the EuRoC~\citep{Burri25012016} dataset.}
    \label{fig:stereo-slam-baseline-perturb-more-cases}
\end{figure}


\begin{figure*}[t]
    \centering
    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results-stereo/MH01_stereoi.pdf}
        \caption{No noise; \textit{MH01} sequence.}
        \label{fig:minipage10}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results-stereo/MH02_stereoi.pdf}
        \caption{No noise; \textit{MH02} sequence.}
        \label{fig:minipage11}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results-stereo/MH03_stereoi.pdf}
        \caption{No noise; \textit{MH03} sequence.}
        \label{fig:minipage12}
    \end{minipage}

    \vspace{0.2cm}

    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results-stereo/MH01_stereoi_0dot001.pdf}
        \caption{$\eta \sim \mathcal{N}(0, 0.001)$; \textit{MH01} sequence.}
        \label{fig:minipage13}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results-stereo/MH02_stereoi_0dot001.pdf}
        \caption{$\eta \sim \mathcal{N}(0, 0.001)$; \textit{MH02} sequence.}
        \label{fig:minipage14}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results-stereo/MH03_stereoi_0dot001.pdf}
        \caption{$\eta \sim \mathcal{N}(0, 0.001)$; \textit{MH03} sequence.}
        \label{fig:minipage15}
    \end{minipage}

    \vspace{0.2cm}

    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results-stereo/MH01_stereoi_0dot01.pdf}
        \caption{$\eta \sim \mathcal{N}(0, 0.01)$; \textit{MH01} sequence.}
        \label{fig:minipage16}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.33\linewidth}
        \centering    
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results-stereo/MH02_stereoi_0dot01_m.pdf}
        \caption{$\eta \sim \mathcal{N}(0, 0.01)$; \textit{MH02} sequence.}
        \label{fig:minipage17}
    \end{minipage}%
    \hfill 
    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/multi-view-qualitative-results-stereo/MH03_stereoi_0dot01.pdf}
        \caption{$\eta \sim \mathcal{N}(0, 0.01)$; \textit{MH03} sequence.}
        \label{fig:minipage18}
    \end{minipage}

    \caption{\textbf{Effect of perturbations on the stereo camera baseline for the ORBSLAM3~\citep{orbslam3} SLAM model with the stereo-inertia input setting.} We introduce a random noise $\eta$ along the axis of the stereo camera baseline. The noise is sampled from a Gaussian distribution with zero mean and variance $\sigma^2$, represented as $\eta \sim \mathcal{N}(0, \sigma^2)$. Here, we show the qualitative comparisons on three sequences of the EuRoC~\citep{Burri25012016} dataset.}
    \label{fig:stereo-slam-baseline-perturb-more-cases-with-imu}
\end{figure*}

==> src/7-aknowledgement.tex <==
\section*{Acknowledgment}
The authors appreciate partial GPU resources provided by Prof. Ram Vasudevan from UMich Robotics. The authors are grateful to Dr. Lu Li from CMU, Prof. Siheng Chen from SJTU, Dr. Wenshan Wang from CMU, and Dr. Youmin Zhang from University of Bologna for valuable discussions. The authors express their gratitude to Prof. Sara Nezami Nav, Prof. Pamela Bogart,   Mrs. Lucy Kates, and Mr. Todd Maslyk from UMich ELI for proofreading.


==> tables/table_benchmarking_methods_bak.tex <==
\begin{table*}[t]
\centering
\caption{SLAM Methods for Robustness Evaluation${}^{\text{(1)}}$.}
\label{tab:slam_methods}
%\centering\setlength{\tabcolsep}{1.4mm}
\resizebox{\textwidth}{!} 
{
\begin{tabular}{l|c|c| l |c|c|r|c|c|c}
\toprule\toprule
\textbf{Method } & \textbf{Type} & \begin{tabular}[c]{@{}c@{}}\textbf{Modality}\\\textbf{Mono/RGBD}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Map} \textbf{Representation}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Loop}\\\textbf{Closure}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{External}\\\textbf{Data}\end{tabular}& \multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Speed${}^{\text{(3)}}$}\end{tabular}} & \textbf{Processing} & \textbf{Year} & \textbf{Repo}\\ 
\midrule 
%VINS-Fusion~\cite{qin2019general} & Classical, Sparse & $\usym{2713}$\quad/\quad$\usym{2713}$ & Feature points, Explicit &$\usym{2713}$ & Real-time & CPU & 2019 &\cite{VINS-Fusion-Repo}\\
ORB-SLAM3~\cite{orbslam3}  & Classical, Sparse & $\usym{2713}$\quad/\quad$\usym{2713}$ & Keyframe+ORB, Explicit  &$\usym{2713}$ &  $\usym{2715}$& Real-time & CPU & 2020 &\cite{ORB-SLAM3-Repo}\\
iMAP~\cite{imap}  & Neural, Dense  &  $\usym{2715}$\quad/\quad$\usym{2713}$ & NeRF-based${}^{\text{(2)}}$, Implicit &$\usym{2715}$ &  $\usym{2715}$ & Not Real-time & CPU+GPU & 2021  & \cite{NICE-SLAM-Repo}\\
Nice-SLAM~\cite{niceslam}  & Neural, Dense & $\usym{2715}$\quad/\quad$\usym{2713}$ & NeRF-based, Implicit &$\usym{2715}$ &  $\usym{2715}$& Not Real-time & CPU+GPU & 2022 & \cite{NICE-SLAM-Repo} \\
CO-SLAM~\cite{coslam}  & Neural, Dense & $\usym{2715}$\quad/\quad$\usym{2713}$ & NeRF-based, Implicit &$\usym{2715}$ &  $\usym{2715}$ & Real-time & CPU+GPU & 2023 & \cite{Co-SLAM-Repo} \\
GO-SLAM~\cite{zhang2023goslam}  & Neural, Dense & $\usym{2713}$\quad/\quad$\usym{2713}$ & NeRF-based, Implicit &$\usym{2713}$ &  $\usym{2713}$${}^{\text{(4)}}$& Quasi Real-time & CPU+GPU & 2023 & \cite{GO-SLAM-Repo} \\
SplaTAM-S~\cite{keetha2023splatam}  & Neural, Dense & $\usym{2715}$\quad/\quad$\usym{2713}$  & Gaussian~\cite{gaussiansplatting}, Explicit &$\usym{2715}$ &  $\usym{2715}$& Quasi Real-time & CPU+GPU & 2023 & \cite{SplaTAM-Repo} \\
\bottomrule\bottomrule
\multicolumn{9}{l}{{$(1)$ We only select several representative SLAM models with varied properties for evaluation in this work.}}\\
\multicolumn{9}{l}{{$(2)$ NeRF-based indicates methods that leverage implicit neural networks to encode the 3D scene, following the philosophy of NeRF~\cite{rosinol2022nerf}.}}\\
\multicolumn{9}{l}{{$(3)$ For the speed comparison, 'Real-time', 'Quasi Real-time', and 'Not Real-time' are in the speed decreasing rank.}}\\
\multicolumn{9}{l}{{$(4)$ GO-SLAM initializes the model parameters from the DROID-SLAM model~\cite{teed2021droid} which leverages external dataset~\cite{wang2020tartanair} for model pre-training.}}\\
\end{tabular}}

\end{table*}% Map Representation

==> tables/table_dataset_compare.tex <==
\begin{table}[t]\vspace{-1mm}
\caption{Synthetic RGB-D SLAM benchmark comparison.}
\centering 
\label{tab:datasets}
\setlength{\tabcolsep}{3pt}
\resizebox{0.48\textwidth}{!}
{
\begin{tabular}{l|r|r|cccc|c}
\toprule

\multirow{2}{*}{{\textbf{Benchmark}}} &
  \multirow{2}{*}{{\textbf{\#Seq}}}   &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{\#Perturb}\\ \textbf{Setting}\end{tabular} }    & \multicolumn{4}{c|}{{\textbf{Perturbation Category}}}  &  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Editable}\end{tabular} }  % &
 
 \\ \cmidrule{4-7} %
 &
   &     &  
  {RGB}  &
  {Motion} &
  {Depth} &
  {Sync.} &
  {} 
 \\  %
 \midrule
Replica & 8  & 0   &   \textcolor{red}{\ding{55}} &   \textcolor{red}{\ding{55}} &   \textcolor{red}{\ding{55}} &   \textcolor{red}{\ding{55}} &   \textcolor{red}{\ding{55}}\\ %\midrule
TartanAir & 30   &   \begin{tabular}[c]{@{}c@{}}8\end{tabular}   &  \textcolor[rgb]{0,0.6875,0.3125}{\ding{51}} &   \textcolor[rgb]{0,0.6875,0.3125}{\ding{51}}&   \textcolor{red}{\ding{55}} &   \textcolor{red}{\ding{55}} &   \textcolor{red}{\ding{55}} \\ %\midrule
\begin{tabular}[c]{@{}c@{}}{\textbf{\textit{Grand-SLAM}}} \end{tabular} & {\textbf{{1,000}}}   & \begin{tabular}[c]{@{}c@{}}\textbf{124} \end{tabular}    &   \textcolor[rgb]{0,0.6875,0.3125}{\ding{51}} &   \textcolor[rgb]{0,0.6875,0.3125}{\ding{51}} &   \textcolor[rgb]{0,0.6875,0.3125}{\ding{51}} &   \textcolor[rgb]{0,0.6875,0.3125}{\ding{51}} &   \textcolor[rgb]{0,0.6875,0.3125}{{\ding{51}}} 
  \\ \bottomrule
\end{tabular}}%\vspace{-2mm}
\end{table}  

% Replica~\citep{straub2019replica}  TartanAir~\citep{wang2020tartanair} 

==> tables/table_dataset_compare_bak.tex <==
\begin{table*}[h!]
%\vspace*{0.5cm} 
\caption{Comparison of SLAM datasets. The table is extended from \cite{helmberger2022hilti}.}
%\footnote{The table is extended from \cite{helmberger2022hilti}.}
\centering
\label{tab:datasets}
\begin{tabular}{ccccccc}
\hline \hline
\textbf{Dataset} &
  \textbf{Num. seq,} &
  \textbf{Environment} &
  \textbf{Motion} &
  \textbf{Sensors} &
  \textbf{Synchronization} &
  \textbf{Ground truth} \\ \hline \hline
  
EuRoC~\cite{Burri25012016} &
  11 &
  Indoor &
  UAV &
  \begin{tabular}[c]{@{}c@{}}1 Stereo camera\\ 1 IMU\end{tabular} &
  Hw &
  \begin{tabular}[c]{@{}c@{}}Laser tracker,\\ MoCap\end{tabular} \\ \hline
KITTI~\cite{Geiger2012CVPR} &
  22 &
  Outdoor &
  Car &
  \begin{tabular}[c]{@{}c@{}}1 Stereo camera\\ 1 Stereo RGB camera\\ 1 Lidar\\ 1 IMU\end{tabular} &
  Sw &
  GNSS-INS \\ \hline
Malaga~\cite{blanco2014malaga} &
  15 &
  Outdoor &
  Car &
  \begin{tabular}[c]{@{}c@{}}1 Stereo RGB camera\\ 1 IMU\end{tabular} &
  Sw &
  GPS \\ \hline
\begin{tabular}[c]{@{}c@{}}The Newer \\ College Dataset~\cite{zhang2021multi}\end{tabular} &
  3 &
  In- / Outdoor &
  Handheld &
  \begin{tabular}[c]{@{}c@{}}4 Cameras\\ 1 Lidars\\ 2 Imus\end{tabular} &
  Hw / Sw &
  \begin{tabular}[c]{@{}c@{}}3D imaging laser \\ scanner, ICP\end{tabular} \\ \hline
PennCOSYVIO~\cite{pfrommer2017penncosyvio} &
  4 &
  In- / Outdoor &
  Handheld &
  \begin{tabular}[c]{@{}c@{}}4 RGB cameras\\ 1 Stereo camera\\ 1 Fisheye camera\\ 2 IMUs\end{tabular} &
  Hw / Sw &
  \begin{tabular}[c]{@{}c@{}}Fiducial \\ markers\end{tabular} \\ \hline
TartanAir~\cite{tartanair2020iros} &
  30 &
  In- / Outdoor &
  Simulation &
  \begin{tabular}[c]{@{}c@{}}Synthetic \\ 1 stereo RGB camera\end{tabular} &
  Sim. &
  Simulation \\ \hline
TUM VIO~\cite{schubert2018tum} &
  28 &
  In- / Outdoor &
  Handheld &
  \begin{tabular}[c]{@{}c@{}}1 Stereo camera\\ 1 IMU\end{tabular} &
  Hw &
  \begin{tabular}[c]{@{}c@{}}MoCap \\ (start, end)\end{tabular} \\ \hline
UMA VI~\cite{zuniga2020vi} &
  32 &
  In- / Outdoor &
  Handheld &
  \begin{tabular}[c]{@{}c@{}}1 Stereo RGB camera\\ 1 Stereo camera\\ 1 IMU\end{tabular} &
  Hw &
  \begin{tabular}[c]{@{}c@{}}Pose alignment\\ (start, end)\end{tabular} \\ \hline
UMich~\cite{carlevaris2016university} &
  27 &
  In- / Outdoor &
  UGV &
  \begin{tabular}[c]{@{}c@{}}6 RGB cameras\\ 1 IMU\end{tabular} &
  Sw &
  \begin{tabular}[c]{@{}c@{}}Fusion of GPS, \\ IMU, laser\end{tabular} \\ \hline
UZH-FPV~\cite{Delmerico19icra} &
  28 &
  In- / Outdoor &
  UAV &
  \begin{tabular}[c]{@{}c@{}}1 Stereo camera\\ 1 Event camera\\ 2 IMUs\end{tabular} &
  Hw / Sw &
  \begin{tabular}[c]{@{}c@{}}Fusion of vision,\\ IMU, laser\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}Hilti~\cite{helmberger2022hilti}\end{tabular} &
  12 &   
  In- / Outdoor &
  Handheld &
  \begin{tabular}[c]{@{}c@{}}5 Cameras\\ 2 Lidars\\ 3 Imus\end{tabular} &
  Hw / Sw &
  \begin{tabular}[c]{@{}c@{}}MoCap, \\ Total Station\end{tabular} \\ \hline
    Campus-Hybrid~\cite{tian2023resilient}   & 3 &  In- / Outdoor  &  UGV &  \begin{tabular}[c]{@{}c@{}} 1 Camera\\ 1 Lidar \\ 1 Imu\end{tabular} &
  xxx & \begin{tabular}[c]{@{}c@{}} Fusion of station,\\ IMU, GPS, laser\end{tabular}
   
   \\ \hline 
     \begin{tabular}[c]{@{}c@{}}\textcolor{red}{[TO Supplement] DARPA} \\ Subterranean~\cite{SubT}\end{tabular}  & x &  Indoor &  Multi- &  \begin{tabular}[c]{@{}c@{}}x Cameras\\ x Lidars\\ x Imus\end{tabular} &
  xxx & \begin{tabular}[c]{@{}c@{}} Fusion of vision,\\ IMU, laser\end{tabular}
   
   \\ \hline  \hline
   
\begin{tabular}[c]{@{}c@{}}\textbf{RobuSLAM} \\\textbf{Dataset} (\textbf{Ours})\end{tabular} &
  \textcolor{black}{\textbf{$>$2,000}} &
  In- / Outdoor &
   \begin{tabular}[c]{@{}c@{}} Random,  \textbf{Diverse}\\ \textbf{robot locomotion}, \\ (\textit{e.g.}, car, rolling robot, \\ and legged robot) \end{tabular}  &
  \begin{tabular}[c]{@{}c@{}} Synthetic \textbf{Multiple}- \\Stereo Cameras \\ RGBD Cameras \\ Imus \end{tabular} &
  Sim. &
  \begin{tabular}[c]{@{}c@{}}Simulation\end{tabular}
  \\ \hline 
  \begin{tabular}[c]{@{}c@{}}\textbf{RobuSLAM} \\\textbf{Simulator} (\textbf{Ours})\end{tabular} &
  \textcolor{black}{\textbf{Infinity}} &
  In- / Outdoor &
   \begin{tabular}[c]{@{}c@{}} Random,  \textbf{Diverse}\\ \textbf{robot locomotion}, \\ (\textit{e.g.}, car, rolling robot, \\ and legged robot) \end{tabular}  &
  \begin{tabular}[c]{@{}c@{}} Synthetic \textbf{Multiple}- \\Stereo Cameras \\ RGBD Cameras \\ Imus, Lidars \end{tabular} &
  Sim. &
  \begin{tabular}[c]{@{}c@{}}Simulation\end{tabular}
  \\ \hline \hline
\end{tabular}
\end{table*}

==> tables/table_make_figure.tex <==
\begin{table}[t]

    \centering
    \setlength{\tabcolsep}{2.5mm}
    \caption{Trajectory estimation error (ATE [m]) of monocular (\textbf{Top}) and RGBD (\textbf{Bottom}) SLAM under faster motion.}%\vspace{-3mm}
        \label{tab:faster-motion-perturbation}
\resizebox{0.48\textwidth}{!}
{
\begin{tabular}{l|c|ccc}
    \toprule \toprule
     {\textbf{Speed-up Ratio}}
     & {$\textbf{1}\times$} & \textbf{$\textbf{2}\times$} & \textbf{$\textbf{4}\times$} & \textbf{$\textbf{8}\times$}    \\ \midrule 
    GO-SLAM (Mono)~\cite{zhang2023goslam} & $\textbf{0.0039}$ & $\textbf{{0.0042}}$ & $\textbf{{0.0046}}$ & $\textbf{{0.0048}}$ 
    \\
    \midrule %\midrule
    iMAP (RGBD)~\cite{imap}& $0.1209$ & $0.4675$ & $0.9445$ & $${1.0000}$$ 
    \\
    Nice-SLAM (RGBD)~\cite{niceslam} & $0.0147$ & $0.1702$ & $${1.0000}$$ & $${1.0000}$$  
    \\
    CO-SLAM (RGBD)~\cite{coslam}& $0.0090$ & $0.1062$ & $0.9510$ & $${1.0000}$$ 
    \\
    GO-SLAM (RGBD)~\cite{zhang2023goslam} & ${0.0046}$ & $\textbf{{0.0046}}$ & $\textbf{{0.0046}}$ & $\textbf{{0.0050}}$  
    \\
SplaTAM-S (RGBD)~\cite{keetha2023splatam}& $\textbf{0.0045}$ & $0.0184$ & $${1.0000}$$ & $${1.0000}$$ 
    \\
    \bottomrule \bottomrule
  \multicolumn{5}{l}{{\textbf{1}) Notice that the sensor stream under faster motion effect is synthesized}}  \\
  \multicolumn{5}{l}{{ by downsampling the original sensor stream. Thus, the derived sensor stream}}\\
     \multicolumn{5}{l}{{ under faster motion is shorter than the original one.}} \\

    \end{tabular}% Models with the best performance are in \textbf{bold}
    
}\end{table}




\begin{table}[t]
\caption{Trajectory estimation error (ATE [m]) under {depth imaging perturbation} for RGBD SLAM methods. }
\label{tab:depth-perturb}
\centering 
\setlength{\tabcolsep}{0.6mm}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|c|cccc}
    \toprule \toprule   
    \multirow{2}{*}{\textbf{Method}} &    \multirow{2}{*}{\textbf{Clean}}
     &  {\textbf{Gaussian}}   & {\textbf{Edge}} & 
  {\textbf{Random}}  & {\textbf{Range}}      \\  
 & & \textbf{Noise} & \textbf{Erosion} & \textbf{Missing} & \textbf{Clipping}\\ \midrule
    iMAP (RGBD)~\cite{imap} & $0.1209$ & $${1.0000}$$ & $0.0307$ & $0.1083$  & $0.2438$ 
    \\ 
    Nice-SLAM (RGBD)~\cite{niceslam}& $0.0147$ & $${1.0000}$$ & $0.0149$ & $0.0154$  & $0.1183$ 
    \\
    CO-SLAM (RGBD)~\cite{coslam}& $0.0090$ & $0.5794$ & $0.0096$ & $0.0094$  & $0.0122$ 
    \\
    GO-SLAM (RGBD)~\cite{zhang2023goslam} & ${0.0046}$ & $\textbf{0.0378}$ & $0.0046$ & ${0.0046}$ & $\textbf{{0.0045}}$   
    \\
    SplaTAM-S (RGBD)~\cite{keetha2023splatam}& $\textbf{0.0045}$ & $${1.0000}$$ & $\textbf{{0.0042}}$ & $\textbf{0.0042}$  
  & ${0.0048}$ 
    \\
    \bottomrule \bottomrule
    \multicolumn{6}{l}{{$${1.0000}$$ indicates  completely unacceptable trajectory estimation performance,}} \\
        \multicolumn{6}{l}{{\textit{i.e.}, ATE $\geq$ 1.0 [m]. Models with the best performance are in \textbf{bold}}}
    \end{tabular}
}
 
\end{table}




\begin{table*}[th]
    \centering

       \caption{Trajectory estimation error (ATE [m]) under trajectory-level deviation.}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccc|cccc|cccc|cccc}
    \toprule \toprule
     \textbf{Rotate [$\deg$]} & \multirow{2}{*}{\textbf{Clean}}  & \multicolumn{3}{c|}{\textbf{\textit{0}}} & \multicolumn{4}{c|}{\textbf{\textit{1}}} & \multicolumn{4}{c|}{\textbf{\textit{3}}} & \multicolumn{4}{c}{\textbf{\textit{5}}}
    \\ \cmidrule{1-1} \cmidrule{3-5} \cmidrule{6-9} \cmidrule{10-13} \cmidrule{14-17}
     \textbf{Translate  [$m$]} &  & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} & \textit{\textbf{0}} & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} & \textit{\textbf{0}}  & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} & \textit{\textbf{0}} & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} 
    \\\midrule\midrule
    GO-SLAM (Mono)~\cite{zhang2023goslam} & $\textbf{0.0039}$ & $\textbf{0.0084}$ & $\textbf{0.0077}$ & $\textbf{0.0091}$ & $\textbf{0.0083}$ & $\textbf{0.0079}$ & $\textbf{0.0082}$ & $\textbf{0.0094}$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$  
    \\ \midrule
   iMAP (RGBD)~\cite{imap} & $0.1209$ & $0.0334$ & $0.1386$ & $0.0442$ & $0.2438$ & $0.2135$ & $0.3754$ & $0.2801$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$   \\
    Nice-SLAM (RGBD)~\cite{niceslam}& $0.0147$ & $0.5812$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ 
    \\
    CO-SLAM (RGBD)~\cite{coslam}& $0.0090$ & $0.0420$ & $0.0848$ & $0.3087$ & $0.4579$ & $0.5069$ & $0.2998$ & $0.5040$ & $0.6443$ & $0.6630$ & $0.7532$ & $0.5772$ & $0.8457$ & $0.7966$ & $0.8277$ & $${1.0000}$$ 
    \\

    GO-SLAM (RGBD)~\cite{zhang2023goslam} & ${0.0046}$ & $\textbf{0.0082}$ & $\textbf{0.0082}$ & $\textbf{0.0081}$ & $\textbf{0.0080}$ & $\textbf{0.0080}$ & $\textbf{0.0078}$ & $\textbf{0.0077}$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$  
    \\
SplaTAM-S (RGBD)~\cite{keetha2023splatam}& $\textbf{0.0045}$ & $0.0545$ & $0.0980$ & $0.2964$ & $0.297F$ & $0.2272$ & $0.2313$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ % \\
    \\ 

    \bottomrule \bottomrule

          \multicolumn{17}{l}{{Notation  represents settings that include failure sequences where no final trajectory is generated due to tracking loss. The number in front of  represents the}}\\
     \multicolumn{17}{l}{{ average ATE as failure sequences are set as a value of 1.0. Notation $${1.0000}$$ indicates completely unacceptable trajectory estimation performance, \textit{i.e.}, ATE $\geq$ 1.0 [m].  }}\\ 
    \end{tabular}
}
         \label{tab:trajectory-perturbation_sr_metric}
\end{table*}% 








\begin{table*}[t]
\caption{Trajectory estimation error (ATE [m]) under static mode of image perturbations. }
\label{tab:image_perturb}
\centering\setlength{\tabcolsep}{0.4mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cccc|cccc|cccc|cccc}
    \toprule \toprule
   Mean &  Clean  & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    GO-SLAM (Mono)~\cite{zhang2023goslam} & $\textbf{0.0039}$  & $\textbf{0.0151}$ & $\textbf{0.0052}$ & $\textbf{0.0052}$ & $\textbf{0.0089}$ & $\textbf{0.0776}$ & $\textbf{0.0456}$ & $\textbf{0.0296}$ & $\textbf{0.0190}$ & $\textbf{0.2157}$ & $\textbf{0.7207}$ & $\textbf{0.1921}$ & $\textbf{0.0859}$ & $\textbf{0.0046}$ & $\textbf{0.0047}$ & $\textbf{0.0095}$ & $\textbf{0.0046}$ 
   
    \\ 
       % \multicolumn{20}{c}{\textbf{Static Perturbation} Mode for \textbf{RGBD} SLAM Models}  \\ \midrule
    iMAP (RGBD)~\cite{imap} & $0.1209$  & $0.1424$ & $0.1671$ & $0.1811$ & $0.0672$ & $0.0278$ & $0.0779$ & $0.1710$ & $0.1087$ & $0.1913$ & $0.1316$ & $0.1665$ & $0.1473$ & $0.1903$ & $0.3831$ & $0.1884$ & $0.1669$  
    \\
    Nice-SLAM (RGBD)~\cite{niceslam}& $0.0147$  & $0.0307$ & $0.0151$ & $0.0161$ & $0.0188$ & $0.0254$ & $0.0377$ & $0.0353$ & $0.0151$ & $0.0186$ & $0.0160$ & $0.0323$ & $0.0320$ & $0.0654$ & $0.0161$ & $0.0150$ & $0.0145$
    \\
    CO-SLAM (RGBD)~\cite{coslam}& $0.0090$   & $\textbf{0.0115}$ & $0.0096$ & $0.0097$ & $0.0097$ & $0.0125$ & $0.0101$ & $0.0099$ & $0.0105$ & $0.0118$ & $0.0113$ & $0.0104$ & $0.0098$ & $0.0103$ & $0.0112$ & $0.0094$ & $0.0094$

    \\

    GO-SLAM (RGBD)~\cite{zhang2023goslam} & $0.0046$  & $0.0135$ & $\textbf{0.0052}$ & ${0.0052}$ & $0.0090$ & $0.0169$ & $0.0140$ & $0.0171$ & $0.0100$ & $0.1211$ & $0.6271$ & $0.0416$ & $0.0164$ & $0.0047$ & $\textbf{0.0054}$ & $0.0065$ & $0.0050$ 
    \\
    SplaTAM-S (RGBD)~\cite{keetha2023splatam}& $\textbf{0.0045}$  & $0.0160$ & $\textbf{0.0052}$  & $\textbf{0.0049}$ & $\textbf{0.0048}$ & $\textbf{0.0054}$ & $\textbf{0.0050}$ & $\textbf{0.0044}$ & $\textbf{0.0051}$ & $\textbf{0.0085}$ & $\textbf{0.0063}$ & $\textbf{0.0048}$ & $\textbf{0.0051}$ & $\textbf{0.0038}$ & $0.0133$ & $\textbf{0.0044}$ & $\textbf{0.0048}$  
    \\  \midrule
     \midrule

        GO-SLAM (Mono)~\cite{zhang2023goslam} & $\textbf{0.0039}$  & $\textbf{0.0155}$ & $\textbf{0.0065}$   & $\textbf{0.0060}$ & $\textbf{0.0090}$  & $\textbf{0.0509}$ & $\textbf{0.0253}$ & $\textbf{0.0396}$ & $\textbf{0.0158}$ & $\textbf{0.2668}$ & $\textbf{0.7395}$& $\textbf{0.2254}$  & $\textbf{0.0474}$ & $\textbf{0.0066}$ & $\textbf{0.0050}$ & $\textbf{0.0298}$ & $\textbf{0.0044}$ 
    \\
    iMAP (RGBD)~\cite{imap} & $0.1209$ & $0.1243$ & $0.1042$ & $0.2149$  & $0.1221$ & $0.1354$ & $0.1170$ & $0.1967$ & $0.1576$ & $0.2279$ & $0.2873$ & $0.2412$ & $0.1528$ & $0.2141$ & $0.2576$ & $0.1607$ & $0.0955$ 
    \\
    Nice-SLAM (RGBD)~\cite{niceslam}& $0.0147$ & $0.0157$ & $0.0252$ & $0.0359$ & $0.0211$ & $0.0288$ & $0.0409$ & $0.0146$ & $0.0155$ & $0.0167$ & $0.0211$ & $0.0197$ & $0.0187$ & $0.0206$ & $0.0155$ & $0.0146$ & $0.0170$
    \\
    CO-SLAM (RGBD)~\cite{coslam}& $0.0090$  & $\textbf{0.0107}$ & $0.0095$ & $0.0115$ & $0.0093$ & $0.0106$ & $0.0103$ & $0.0102$ & $0.0098$ & $0.0117$ & $0.0116$ & $\textbf{0.0111}$ & $0.0109$ & $0.0106$ & $0.0111$ & $0.0095$ & $0.0097$
    \\
 GO-SLAM (RGBD)~\cite{zhang2023goslam} & $0.0046$  & $0.0130$ & $0.0057$ & $0.0055$ & $0.0078$ & $0.0185$ & $0.0117$ & $0.0139$ & $0.0098$ & $0.1685$ & $0.2213$ & $0.0637$ & $0.0166$ & $\textbf{0.0051}$ & $\textbf{0.0052}$ & $0.0092$ & $0.0049$ 
    \\ 
    SplaTAM-S (RGBD)~\cite{keetha2023splatam}& $\textbf{0.0045}$  & $0.0191$ & $\textbf{0.0053}$  & $\textbf{0.0052}$ & $\textbf{0.0050}$ & $\textbf{0.0058}$ & $\textbf{0.0072}$ & $\textbf{0.0044}$ & $\textbf{0.0067}$ & $\textbf{0.0062}$ & $\textbf{0.0062}$ & $0.045$ & $\textbf{0.0041}$ & $0.0054$ & $0.0096$ & $\textbf{0.0046}$ & $\textbf{0.0045}$  
    \\   
    \bottomrule  \bottomrule

    \end{tabular}
}
\end{table*}






\begin{table*}[t]
\caption{Trajectory estimation error (ATE [m]) under static mode of image perturbations. }
\label{tab:image_perturb}
\centering\setlength{\tabcolsep}{0.4mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cccc|cccc|cccc|cccc}
    \toprule \toprule
   Mean &  Clean  & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    GO-SLAM (Mono)~\cite{zhang2023goslam} & $\textbf{0.0039}$  & $\textbf{0.0151}$ & $\textbf{0.0052}$ & $\textbf{0.0052}$ & $\textbf{0.0089}$ & $\textbf{0.0776}$ & $\textbf{0.0456}$ & $\textbf{0.0296}$ & $\textbf{0.0190}$ & $\textbf{0.2157}$ & $\textbf{0.7207}$ & $\textbf{0.1921}$ & $\textbf{0.0859}$ & $\textbf{0.0046}$ & $\textbf{0.0047}$ & $\textbf{0.0095}$ & $\textbf{0.0046}$ 
   
    \\ 
       % \multicolumn{20}{c}{\textbf{Static Perturbation} Mode for \textbf{RGBD} SLAM Models}  \\ \midrule
    iMAP (RGBD)~\cite{imap} & $0.1209$  & $0.1424$ & $0.1671$ & $0.1811$ & $0.0672$ & $0.0278$ & $0.0779$ & $0.1710$ & $0.1087$ & $0.1913$ & $0.1316$ & $0.1665$ & $0.1473$ & $0.1903$ & $0.3831$ & $0.1884$ & $0.1669$  
    \\
    Nice-SLAM (RGBD)~\cite{niceslam}& $0.0147$  & $0.0307$ & $0.0151$ & $0.0161$ & $0.0188$ & $0.0254$ & $0.0377$ & $0.0353$ & $0.0151$ & $0.0186$ & $0.0160$ & $0.0323$ & $0.0320$ & $0.0654$ & $0.0161$ & $0.0150$ & $0.0145$
    \\
    CO-SLAM (RGBD)~\cite{coslam}& $0.0090$   & $\textbf{0.0115}$ & $0.0096$ & $0.0097$ & $0.0097$ & $0.0125$ & $0.0101$ & $0.0099$ & $0.0105$ & $0.0118$ & $0.0113$ & $0.0104$ & $0.0098$ & $0.0103$ & $0.0112$ & $0.0094$ & $0.0094$

    \\

    GO-SLAM (RGBD)~\cite{zhang2023goslam} & $0.0046$  & $0.0135$ & $\textbf{0.0052}$ & ${0.0052}$ & $0.0090$ & $0.0169$ & $0.0140$ & $0.0171$ & $0.0100$ & $0.1211$ & $0.6271$ & $0.0416$ & $0.0164$ & $0.0047$ & $\textbf{0.0054}$ & $0.0065$ & $0.0050$ 
    \\
    SplaTAM-S (RGBD)~\cite{keetha2023splatam}& $\textbf{0.0045}$  & $0.0160$ & $\textbf{0.0052}$  & $\textbf{0.0049}$ & $\textbf{0.0048}$ & $\textbf{0.0054}$ & $\textbf{0.0050}$ & $\textbf{0.0044}$ & $\textbf{0.0051}$ & $\textbf{0.0085}$ & $\textbf{0.0063}$ & $\textbf{0.0048}$ & $\textbf{0.0051}$ & $\textbf{0.0038}$ & $0.0133$ & $\textbf{0.0044}$ & $\textbf{0.0048}$  
    \\ 
    \bottomrule  \bottomrule

    \end{tabular}
}
\end{table*}


\begin{table*}[t]
\caption{Trajectory estimation error (ATE [m]) under Dynamic mode of image perturbations. }
\label{tab:image_perturb}
\centering\setlength{\tabcolsep}{0.4mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cccc|cccc|cccc|cccc}
    \toprule \toprule
   Mean &  Clean  & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contrast} & \textbf{JPEG}  & \textbf{Pixelate}
    \\\midrule\midrule

        GO-SLAM (Mono)~\cite{zhang2023goslam} & $\textbf{0.0039}$  & $\textbf{0.0155}$ & $\textbf{0.0065}$   & $\textbf{0.0060}$ & $\textbf{0.0090}$  & $\textbf{0.0509}$ & $\textbf{0.0253}$ & $\textbf{0.0396}$ & $\textbf{0.0158}$ & $\textbf{0.2668}$ & $\textbf{0.7395}$& $\textbf{0.2254}$  & $\textbf{0.0474}$ & $\textbf{0.0066}$ & $\textbf{0.0050}$ & $\textbf{0.0298}$ & $\textbf{0.0044}$ 
    \\
    iMAP (RGBD)~\cite{imap} & $0.1209$ & $0.1243$ & $0.1042$ & $0.2149$  & $0.1221$ & $0.1354$ & $0.1170$ & $0.1967$ & $0.1576$ & $0.2279$ & $0.2873$ & $0.2412$ & $0.1528$ & $0.2141$ & $0.2576$ & $0.1607$ & $0.0955$ 
    \\
    Nice-SLAM (RGBD)~\cite{niceslam}& $0.0147$ & $0.0157$ & $0.0252$ & $0.0359$ & $0.0211$ & $0.0288$ & $0.0409$ & $0.0146$ & $0.0155$ & $0.0167$ & $0.0211$ & $0.0197$ & $0.0187$ & $0.0206$ & $0.0155$ & $0.0146$ & $0.0170$
    \\
    CO-SLAM (RGBD)~\cite{coslam}& $0.0090$  & $\textbf{0.0107}$ & $0.0095$ & $0.0115$ & $0.0093$ & $0.0106$ & $0.0103$ & $0.0102$ & $0.0098$ & $0.0117$ & $0.0116$ & $\textbf{0.0111}$ & $0.0109$ & $0.0106$ & $0.0111$ & $0.0095$ & $0.0097$
    \\
 GO-SLAM (RGBD)~\cite{zhang2023goslam} & $0.0046$  & $0.0130$ & $0.0057$ & $0.0055$ & $0.0078$ & $0.0185$ & $0.0117$ & $0.0139$ & $0.0098$ & $0.1685$ & $0.2213$ & $0.0637$ & $0.0166$ & $\textbf{0.0051}$ & $\textbf{0.0052}$ & $0.0092$ & $0.0049$ 
    \\ 
    SplaTAM-S (RGBD)~\cite{keetha2023splatam}& $\textbf{0.0045}$  & $0.0191$ & $\textbf{0.0053}$  & $\textbf{0.0052}$ & $\textbf{0.0050}$ & $\textbf{0.0058}$ & $\textbf{0.0072}$ & $\textbf{0.0044}$ & $\textbf{0.0067}$ & $\textbf{0.0062}$ & $\textbf{0.0062}$ & $0.045$ & $\textbf{0.0041}$ & $0.0054$ & $0.0096$ & $\textbf{0.0046}$ & $\textbf{0.0045}$  
    \\   
    \bottomrule  \bottomrule

    \end{tabular}
}
\end{table*}










==> tables/table_mixed_perturbation_bak.tex <==





\begin{wraptable}{r}{0.52\textwidth}
%\begin{table}[t!]
\vspace{-4mm}
\centering
\caption{{{Effect of mixed perturbations on ATE$\downarrow$ (m).}{Cells with darker \colorbox{lightgray}{shades} indicate higher ATE.} }}
\label{tab:mixed_perturbation}
\centering\setlength{\tabcolsep}{0.5mm}
\resizebox{0.52\textwidth}{!}{
\begin{tabular}{l|c|cccccc}
\toprule\toprule

\textbf{Perturbation Type} &\textbf{Clean}& \multicolumn{6}{c}{\textbf{Perturbation Composition}} \\ \midrule
RGB Snow Effect             & &  \checkmark&  \checkmark&  \checkmark                 & \checkmark &\checkmark &\checkmark \\  
RGB Motion Blur     &    &   &  \checkmark&  \checkmark &\checkmark     &  \checkmark                &\checkmark            \\
RGB Gaussian Noise   &&     &  &      \checkmark   &\checkmark  &\checkmark   &          \checkmark   \\
RGB JPEG Compress.  &    && &         & \checkmark  &\checkmark   &\checkmark                \\ 
Depth Gaussian Noise   &  & &  &         &                  &     \checkmark              &   \checkmark                         \\  
RGBD De-sync.  &   &&   &               &                  &                  &                     \checkmark      \\ \midrule
GO-SLAM~\cite{zhang2023goslam} & {0.005}&  \cellcolor{red!12}{0.056} & \cellcolor{red!28}{0.139} & \cellcolor{red!40}{0.196} & \cellcolor{red!26}{0.127}  & \cellcolor{red!42}{0.211} & \cellcolor{red!66}{0.327}                 \\ %\midrule
SplaTAM-S~\cite{keetha2023splatam} & {0.005}&  \cellcolor{red!01}{0.005} & \cellcolor{red!28}{0.007} & \cellcolor{red!40}{0.008} & \cellcolor{red!40}{0.008}  & \cellcolor{red!42}{0.132} & \cellcolor{red!66}{0.307}                 \\ 

%GO-SLAM~\cite{zhang2023goslam}    &  \cellcolor{red!6}{0.0557} & \cellcolor{red!14}{0.1393} & \cellcolor{red!20}{0.1955} & \cellcolor{red!13}{0.1272}  & \cellcolor{red!21}{0.2106} & \cellcolor{red!33}{0.3274}                 \\ 


\bottomrule\bottomrule
\end{tabular}}
\vspace{-2mm}
%\end{table}
\end{wraptable}
% %ORB-SLAM3~\cite{orbslam3}   & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$                              \\ 
%SplaTAM-S~\cite{keetha2023splatam}    & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$              \\ 
%Goslam:{'14_3_4_3': 0.13926349999999998, '14_3_4_3_6_3': 0.19550699999999996, '14_3_4_3_6_3_15_3': 0.12723, '14_3_4_3_6_3_15_3_18_10': 0.21063049999999997, '14_3_4_3_6_3_15_3_18_10_20_3': 0.32737875, '14_3': 0.055721142857142865}


==> tables/table_sensor_mialign_performance_ablate_goslam.tex <==
\begin{table}[t]
%\begin{wraptable}{r}{0.5\textwidth}
%\vspace{-4mm}
\caption{Effect of global bundle adjustment (GBA) on GO-SLAM under de-synchronization.}
\label{tab:sensor-misalign-perturb}
\centering 
\setlength{\tabcolsep}{0.8mm}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|c|ccc|ccc}
    \toprule \toprule
     \multirow{2}{*}{\textbf{Method}} & \textbf{Clean} &  \multicolumn{3}{c|}{\textbf{Static Mode}}& \multicolumn{3}{c}{\textbf{Dynamic Mode}} \\ \cmidrule{2-5} \cmidrule{6-8}
     & \textbf{$\Delta=0$} & \textbf{$\Delta=5$} & \textbf{$\Delta=10$} & \textbf{$\Delta=20$} & \textbf{$\Delta=5$} & \textbf{$\Delta=10$} & \textbf{$\Delta=20$}      \\ \midrule
  %      \multicolumn{8}{c}{RGB-D Setting}  \\ \midrule
  %  VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$   \\
 %   ORB-SLAM3~\cite{orbslam3} & $0.0823$ & $0.0689$ & $0.0661$  & $0.0647$ & $0.0703$ & $0.0773$ & $0.0826$    \\

   w/ GBA & \textbf{$\textbf{0.0046}$} & \textbf{${\textbf{0.0148}}$} & \textbf{${\textbf{0.0292}}$} & \textbf{${\textbf{0.0646}}$}  & \textbf{{${\textbf{0.0151}}$}} & \textbf{{${\textbf{0.0297}}$}} & {${\textbf{0.0650}}$} 
    \\
    w/o GBA & $0.0052$ & ${0.0183}$ & ${0.0343}$ & ${0.0809}$  & {${0.0186}$} & {${0.0345}$} & {${0.0808}$} 
    \\    
    \bottomrule  \bottomrule
      \multicolumn{8}{l}{{  $\Delta$ denotes the misaligned frame interval between RGB and depth. }}\\
  %  \multicolumn{8}{l}{{\textbf{2}) We highlight the best performance, \textit{i.e.}, the lowest ATE, under each }}\\
   % \multicolumn{8}{l}{{ severity level of multi-sensor misalignment in \textbf{bold}.}}
    \end{tabular}
}%\vspace{-4mm}
\end{table}
%\end{wraptable}

==> tables/table_sensor_perturb_performance_all.tex <==

\begin{table*}[t]
\caption{Per-scene Sensor-level perturbation benchmarking (ATE) on Replica (office0)}

\label{tab:sensor_perturb_benchmark}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|cccc|cccc|cccc}
    \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Mean}} & \multicolumn{5}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Weather Effect}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{3-7} \cmidrule{8-11} \cmidrule{12-15} \cmidrule{16-19}
    &  & \textbf{Zoom} & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{18}{c}{Monocular Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\ \midrule
        \multicolumn{18}{c}{RGBD Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule
    \end{tabular}
}
\end{table*}



\begin{table*}[t]
\caption{Per-scene Sensor-level perturbation benchmarking (ATE) on Replica (office1)}

\label{tab:sensor_recon}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|cccc|cccc|cccc}
    \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Mean}} & \multicolumn{5}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Weather Effect}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{3-7} \cmidrule{8-11} \cmidrule{12-15} \cmidrule{16-19}
    &  & \textbf{Zoom} & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{18}{c}{Monocular Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\ \midrule
        \multicolumn{18}{c}{RGBD Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule
    \end{tabular}
}
\end{table*}



\begin{table*}[t]
\caption{Per-scene Sensor-level perturbation benchmarking (ATE) on Replica (office2)}

\label{tab:sensor_recon}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|cccc|cccc|cccc}
    \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Mean}} & \multicolumn{5}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Weather Effect}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{3-7} \cmidrule{8-11} \cmidrule{12-15} \cmidrule{16-19}
    &  & \textbf{Zoom} & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{18}{c}{Monocular Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\ \midrule
        \multicolumn{18}{c}{RGBD Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule
    \end{tabular}
}
\end{table*}



\begin{table*}[t]
\caption{Per-scene Sensor-level perturbation benchmarking (ATE) on Replica (office3)}

\label{tab:sensor_recon}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|cccc|cccc|cccc}
    \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Mean}} & \multicolumn{5}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Weather Effect}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{3-7} \cmidrule{8-11} \cmidrule{12-15} \cmidrule{16-19}
    &  & \textbf{Zoom} & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{18}{c}{Monocular Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\ \midrule
        \multicolumn{18}{c}{RGBD Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule
    \end{tabular}
}
\end{table*}

\begin{table*}[t]
\caption{Per-scene Sensor-level perturbation benchmarking (ATE) on Replica (office4)}

\label{tab:sensor_recon}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|cccc|cccc|cccc}
    \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Mean}} & \multicolumn{5}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Weather Effect}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{3-7} \cmidrule{8-11} \cmidrule{12-15} \cmidrule{16-19}
    &  & \textbf{Zoom} & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{18}{c}{Monocular Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\ \midrule
        \multicolumn{18}{c}{RGBD Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule
    \end{tabular}
}
\end{table*}


\begin{table*}[t]
\caption{Per-scene Sensor-level perturbation benchmarking (ATE) on Replica (room0)}

\label{tab:sensor_recon}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|cccc|cccc|cccc}
    \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Mean}} & \multicolumn{5}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Weather Effect}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{3-7} \cmidrule{8-11} \cmidrule{12-15} \cmidrule{16-19}
    &  & \textbf{Zoom} & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{18}{c}{Monocular Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\ \midrule
        \multicolumn{18}{c}{RGBD Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule
    \end{tabular}
}
\end{table*}





\begin{table*}[t]
\caption{Per-scene Sensor-level perturbation benchmarking (ATE) on Replica (room1)}

\label{tab:sensor_recon}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|cccc|cccc|cccc}
    \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Mean}} & \multicolumn{5}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Weather Effect}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{3-7} \cmidrule{8-11} \cmidrule{12-15} \cmidrule{16-19}
    &  & \textbf{Zoom} & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{18}{c}{Monocular Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\ \midrule
        \multicolumn{18}{c}{RGBD Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule
    \end{tabular}
}
\end{table*}


\begin{table*}[t]
\caption{Per-scene Sensor-level perturbation benchmarking (ATE) on Replica (room2)}

\label{tab:sensor_recon}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|cccc|cccc|cccc}
    \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Mean}} & \multicolumn{5}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Weather Effect}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{3-7} \cmidrule{8-11} \cmidrule{12-15} \cmidrule{16-19}
    &  & \textbf{Zoom} & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{18}{c}{Monocular Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\ \midrule
        \multicolumn{18}{c}{RGBD Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule
    \end{tabular}
}
\end{table*}





==> tables/table_sensor_perturb_performance_backup_0529.tex <==
\newcommand{\colorcellpurple}[1]{%
  \ifdim #1 pt > 0.0066pt % Threshold 1
    \cellcolor{purple!50}{#1}
    \else
      \ifdim #1 pt > 0.0059 pt % Threshold 3
        \cellcolor{purple!30}{#1}
      \else  
        \ifdim #1 pt > 0.0049 pt % Threshold 4 
          \cellcolor{purple!10}{#1}
        \else
          #1 % No color if below all thresholds
        \fi
      \fi

  \fi
}
\newcommand{\colorcell}[1]{%
  \ifdim #1 pt > 0.018pt % Threshold 1
    \cellcolor{red!50}{#1}

    \else
      \ifdim #1 pt > 0.014 pt % Threshold 3
        \cellcolor{red!30}{#1}
      \else  
        \ifdim #1 pt > 0.010 pt % Threshold 4 
          \cellcolor{red!10}{#1}
        \else
          #1 % No color if below all thresholds
        \fi
      \fi

  \fi
}


\newcommand{\colorcelliMAP}[1]{%
  \ifdim #1 pt > 0.018pt % Threshold 1
    \cellcolor{red!50}{#1}

    \else
      \ifdim #1 pt > 0.014 pt % Threshold 3
        \cellcolor{red!30}{#1}
      \else  
        \ifdim #1 pt > 0.010 pt % Threshold 4 
          \cellcolor{red!10}{#1}
        \else
          #1 % No color if below all thresholds
        \fi
      \fi

  \fi
}

\newcommand{\colorcellMono}[1]{%
  \ifdim #1 pt > 0.018pt % Threshold 1
    \cellcolor{red!50}{#1}

    \else
      \ifdim #1 pt > 0.014 pt % Threshold 3
        \cellcolor{red!30}{#1}
      \else  
        \ifdim #1 pt > 0.010 pt % Threshold 4 
          \cellcolor{red!10}{#1}
        \else
          #1 % No color if below all thresholds
        \fi
      \fi

  \fi
}


\newcommand{\colorcellNice}[1]{%
  \ifdim #1 pt > 0.018pt % Threshold 1
    \cellcolor{red!50}{#1}

    \else
      \ifdim #1 pt > 0.014 pt % Threshold 3
        \cellcolor{red!30}{#1}
      \else  
        \ifdim #1 pt > 0.010 pt % Threshold 4 
          \cellcolor{red!10}{#1}
        \else
          #1 % No color if below all thresholds
        \fi
      \fi

  \fi
}

\newcommand{\colorcellCO}[1]{%
  \ifdim #1 pt > 0.018pt % Threshold 1
    \cellcolor{red!50}{#1}

    \else
      \ifdim #1 pt > 0.014 pt % Threshold 3
        \cellcolor{red!30}{#1}
      \else  
        \ifdim #1 pt > 0.010 pt % Threshold 4 
          \cellcolor{red!10}{#1}
        \else
          #1 % No color if below all thresholds
        \fi
      \fi

  \fi
}

\newcommand{\colorcellGOSLAMRGBD}[1]{%
  \ifdim #1 pt > 0.018pt % Threshold 1
    \cellcolor{red!50}{#1}

    \else
      \ifdim #1 pt > 0.014 pt % Threshold 3
        \cellcolor{red!30}{#1}
      \else  
        \ifdim #1 pt > 0.010 pt % Threshold 4 
          \cellcolor{red!10}{#1}
        \else
          #1 % No color if below all thresholds
        \fi
      \fi

  \fi
}

\newcommand{\colorcellSplaTAM}[1]{%
  \ifdim #1 pt > 0.018pt % Threshold 1
    \cellcolor{red!50}{#1}

    \else
      \ifdim #1 pt > 0.014 pt % Threshold 3
        \cellcolor{red!30}{#1}
      \else  
        \ifdim #1 pt > 0.010 pt % Threshold 4 
          \cellcolor{red!10}{#1}
        \else
          #1 % No color if below all thresholds
        \fi
      \fi

  \fi
}

\begin{table*}[t]
\caption{Trajectory estimation error (ATE$\downarrow$ (m)) under static (\textbf{Top}) and dynamic (\textbf{Bottom}) image perturbations for Neural SLAM models. \xxh{Cells exhibiting a darker coloration indicate higher ATE.} }
\label{tab:image_perturb}
\centering\setlength{\tabcolsep}{0.4mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cc|cccc|cccc|cccc|cccc}
    \toprule \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Clean}}&  \multicolumn{2}{|c|}{\textbf{Perturbed}}  & \multicolumn{4}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Environmental Interference}}  & \multicolumn{4}{c}{\textbf{Post-processing}} 
    \\ \cmidrule{5-8} \cmidrule{9-12} \cmidrule{13-16} \cmidrule{17-20}
    &  & \textbf{Mean} & \textbf{Max}  & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
GO-SLAM (Mono)~\cite{zhang2023goslam} & $\colorcellMono{0.0039}$ & $\colorcellMono{0.0903}$  & $\colorcellMono{0.7207}$ & $\colorcellMono{0.0151}$ & $\colorcellMono{0.0052}$ & $\colorcellMono{0.0052}$ & $\colorcellMono{0.0089}$ & $\colorcellMono{0.0776}$ & $\colorcellMono{0.0456}$ & $\colorcellMono{0.0296}$ & $\colorcellMono{0.0190}$ & $\colorcellMono{0.2157}$ & $\colorcellMono{0.7207}$ & $\colorcellMono{0.1921}$ & $\colorcellMono{0.0859}$ & $\colorcellMono{0.0046}$ & $\colorcellMono{0.0047}$ & $\colorcellMono{0.0095}$ & $\colorcellMono{0.0046}$ \\  \midrule
iMAP (RGBD)~\cite{imap} & $\colorcelliMAP{0.1209}$ & $\colorcelliMAP{0.1568}$ & $\colorcelliMAP{0.3831}$ & $\colorcelliMAP{0.1424}$ & $\colorcelliMAP{0.1671}$ & $\colorcelliMAP{0.1811}$ & $\colorcelliMAP{0.0672}$ & $\colorcelliMAP{0.0278}$ & $\colorcelliMAP{0.0779}$ & $\colorcelliMAP{0.1710}$ & $\colorcelliMAP{0.1087}$ & $\colorcelliMAP{0.1913}$ & $\colorcelliMAP{0.1316}$ & $\colorcelliMAP{0.1665}$ & $\colorcelliMAP{0.1473}$ & $\colorcelliMAP{0.1903}$ & $\colorcelliMAP{0.3831}$ & $\colorcelliMAP{0.1884}$ & $\colorcelliMAP{0.1669}$  \\
Nice-SLAM (RGBD)~\cite{niceslam}& $\colorcellNice{0.0147}$ & $\colorcellNice{0.0253}$ & $\colorcellNice{0.0654}$  & $\colorcellNice{0.0307}$ & $\colorcellNice{0.0151}$ & $\colorcellNice{0.0161}$ & $\colorcellNice{0.0188}$ & $\colorcellNice{0.0254}$ & $\colorcellNice{0.0377}$ & $\colorcellNice{0.0353}$ & $\colorcellNice{0.0151}$ & $\colorcellNice{0.0186}$ & $\colorcellNice{0.0160}$ & $\colorcellNice{0.0323}$ & $\colorcellNice{0.0320}$ & $\colorcellNice{0.0654}$ & $\colorcellNice{0.0161}$ & $\colorcellNice{0.0150}$ & $\colorcellNice{0.0145}$\\
CO-SLAM (RGBD)~\cite{coslam} & $\colorcellCO{0.0090}$ & $\colorcellCO{0.0104}$ &  $\colorcellCO{0.0125}$  & $\colorcellCO{0.0115}$ & $\colorcellCO{0.0096}$ & $\colorcellCO{0.0097}$ & $\colorcellCO{0.0097}$ & $\colorcellCO{0.0125}$ & $\colorcellCO{0.0101}$ & $\colorcellCO{0.0099}$ & $\colorcellCO{0.0105}$ & $\colorcellCO{0.0118}$ & $\colorcellCO{0.0113}$ & $\colorcellCO{0.0104}$ & $\colorcellCO{0.0098}$ & $\colorcellCO{0.0103}$ & $\colorcellCO{0.0112}$ & $\colorcellCO{0.0094}$ & $\colorcellCO{0.0094}$\\

GO-SLAM (RGBD)~\cite{zhang2023goslam} & $\colorcellGOSLAMRGBD{0.0046}$ & $\colorcellGOSLAMRGBD{0.0574}$ &$\colorcellGOSLAMRGBD{0.6271}$ & $\colorcellGOSLAMRGBD{0.0135}$ & $\colorcellGOSLAMRGBD{0.0052}$ & $\colorcellGOSLAMRGBD{0.0052}$ & $\colorcellGOSLAMRGBD{0.0090}$ & $\colorcellGOSLAMRGBD{0.0169}$ & $\colorcellGOSLAMRGBD{0.0140}$ & $\colorcellGOSLAMRGBD{0.0171}$ & $\colorcellGOSLAMRGBD{0.0100}$ & $\colorcellGOSLAMRGBD{0.1211}$ & $\colorcellGOSLAMRGBD{0.6271}$ & $\colorcellGOSLAMRGBD{0.0416}$ & $\colorcellGOSLAMRGBD{0.0164}$ & $\colorcellGOSLAMRGBD{0.0047}$ & $\colorcellGOSLAMRGBD{0.0054}$ & $\colorcellGOSLAMRGBD{0.0065}$ & $\colorcellGOSLAMRGBD{0.0050}$ \\
SplaTAM-S (RGBD)~\cite{keetha2023splatam}& $\colorcellSplaTAM{0.0045}$ & $\colorcellSplaTAM{0.0062}$ & $\colorcellSplaTAM{0.0160}$ & $\colorcellSplaTAM{0.0160}$ & $\colorcellSplaTAM{0.0052}$  & $\colorcellSplaTAM{0.0049}$ & $\colorcellSplaTAM{0.0048}$ & $\colorcellSplaTAM{0.0054}$ & $\colorcellSplaTAM{0.0050}$ & $\colorcellSplaTAM{0.0044}$ & $\colorcellSplaTAM{0.0051}$ & $\colorcellSplaTAM{0.0085}$ & $\colorcellSplaTAM{0.0063}$ & $\colorcellSplaTAM{0.0048}$ & $\colorcellSplaTAM{0.0051}$ & $\colorcellSplaTAM{0.0038}$ & $\colorcellSplaTAM{0.0133}$ & $\colorcellSplaTAM{0.0044}$ & $\colorcellSplaTAM{0.0048}$  \\ 
 
\midrule
        \multicolumn{20}{c}{Optimal performance (min ATE) achieved by using all SLAM models:}  \\ \midrule
      min ATE  & \multirow{3}{*}{$\textbf{0.0039}$} & {{{{0.0056}}}}   & {${0.0115}$} & $0.0115$ & $0.0052$  & $0.0049$ & $0.0048$ & $0.0054$ & $0.0050$ & $0.0044$ & $0.0051$ & $0.0085$ & $0.0063$ & $0.0048$ & $0.0051$ & $0.0038$ & $0.0054$ & $0.0044$ & $0.0046$  
    \\ \cmidrule{5-8}\cmidrule{9-12}\cmidrule{13-16}\cmidrule{17-20}
     mean(min ATE)& & {{\textbf{\colorcellpurple{0.0056}}}}   & {\colorcellpurple{0.0066}}  &  \multicolumn{4}{c|}{\colorcellpurple{0.0066}}&  \multicolumn{4}{c|}{\colorcellpurple{0.0050}}&  \multicolumn{4}{c|}{\colorcellpurple{0.0062}} &  \multicolumn{4}{c}{\colorcellpurple{0.0046}}
    \\ 
       \midrule     \midrule

GO-SLAM (Mono)~\cite{zhang2023goslam} & $\colorcellMono{0.0039}$ & $\colorcellMono{0.0933}$ & $\colorcellMono{0.7395}$ & $\colorcellMono{0.0155}$ & $\colorcellMono{0.0065}$   & $\colorcellMono{0.0060}$ & $\colorcellMono{0.0090}$  & $\colorcellMono{0.0509}$ & $\colorcellMono{0.0253}$ & $\colorcellMono{0.0396}$ & $\colorcellMono{0.0158}$ & $\colorcellMono{0.2668}$ & $\colorcellMono{0.7395}$& $\colorcellMono{0.2254}$  & $\colorcellMono{0.0474}$ & $\colorcellMono{0.0066}$ & $\colorcellMono{0.0050}$ & $\colorcellMono{0.0298}$ & $\colorcellMono{0.0044}$ 
    \\
    \midrule
     %   \multicolumn{20}{c}{\textbf{Dynamic Perturbation} Mode for \textbf{RGBD} SLAM Models}  \\ \midrule
    iMAP (RGBD)~\cite{imap} & $\colorcelliMAP{0.1209}$ & $\colorcelliMAP{0.1756}$ & $\colorcelliMAP{0.2873}$ & $\colorcelliMAP{0.1243}$ & $\colorcelliMAP{0.1042}$ & $\colorcelliMAP{0.2149}$  & $\colorcelliMAP{0.1221}$ & $\colorcelliMAP{0.1354}$ & $\colorcelliMAP{0.1170}$ & $\colorcelliMAP{0.1967}$ & $\colorcelliMAP{0.1576}$ & $\colorcelliMAP{0.2279}$ & $\colorcelliMAP{0.2873}$ & $\colorcelliMAP{0.2412}$ & $\colorcelliMAP{0.1528}$ & $\colorcelliMAP{0.2141}$ & $\colorcelliMAP{0.2576}$ & $\colorcelliMAP{0.1607}$ & $\colorcelliMAP{0.0955}$ 
    \\
    Nice-SLAM (RGBD)~\cite{niceslam}& $\colorcellNice{0.0147}$ & $\colorcellNice{0.0214}$ &$\colorcellNice{0.0409}$ & $\colorcellNice{0.0157}$ & $\colorcellNice{0.0252}$ & $\colorcellNice{0.0359}$ & $\colorcellNice{0.0211}$ & $\colorcellNice{0.0288}$ & $\colorcellNice{0.0409}$ & $\colorcellNice{0.0146}$ & $\colorcellNice{0.0155}$ & $\colorcellNice{0.0167}$ & $\colorcellNice{0.0211}$ & $\colorcellNice{0.0197}$ & $\colorcellNice{0.0187}$ & $\colorcellNice{0.0206}$ & $\colorcellNice{0.0155}$ & $\colorcellNice{0.0146}$ & $\colorcellNice{0.0170}$
    \\
    CO-SLAM (RGBD)~\cite{coslam}& $\colorcellCO{0.0090}$ & $\colorcellCO{0.0105}$ & $\colorcellCO{0.0117}$ & $\colorcellCO{0.0107}$ & $\colorcellCO{0.0095}$ & $\colorcellCO{0.0115}$ & $\colorcellCO{0.0093}$ & $\colorcellCO{0.0106}$ & $\colorcellCO{0.0103}$ & $\colorcellCO{0.0102}$ & $\colorcellCO{0.0098}$ & $\colorcellCO{0.0117}$ & $\colorcellCO{0.0116}$ & $\colorcellCO{0.0111}$ & $\colorcellCO{0.0109}$ & $\colorcellCO{0.0106}$ & $\colorcellCO{0.0111}$ & $\colorcellCO{0.0095}$ & $\colorcellCO{0.0097}$
    \\
 GO-SLAM (RGBD)~\cite{zhang2023goslam} & $\colorcellGOSLAMRGBD{0.0046}$ & $\colorcellGOSLAMRGBD{0.0363}$  & $\colorcellGOSLAMRGBD{0.2213}$ & $\colorcellGOSLAMRGBD{0.0130}$ & $\colorcellGOSLAMRGBD{0.0057}$ & $\colorcellGOSLAMRGBD{0.0055}$ & $\colorcellGOSLAMRGBD{0.0078}$ & $\colorcellGOSLAMRGBD{0.0185}$ & $\colorcellGOSLAMRGBD{0.0117}$ & $\colorcellGOSLAMRGBD{0.0139}$ & $\colorcellGOSLAMRGBD{0.0098}$ & $\colorcellGOSLAMRGBD{0.1685}$ & $\colorcellGOSLAMRGBD{0.2213}$ & $\colorcellGOSLAMRGBD{0.0637}$ & $\colorcellGOSLAMRGBD{0.0166}$ & $\colorcellGOSLAMRGBD{0.0051}$ & $\colorcellGOSLAMRGBD{0.0052}$ & $\colorcellGOSLAMRGBD{0.0092}$ & $\colorcellGOSLAMRGBD{0.0049}$ 
    \\ 
    SplaTAM-S (RGBD)~\cite{keetha2023splatam}& $\colorcellSplaTAM{0.0045}$ & $\colorcellSplaTAM{0.008}$\textit{\textbf{G}} & $\colorcellSplaTAM{0.045}$\textit{\textbf{G}} & $\colorcellSplaTAM{0.0191}$ & $\colorcellSplaTAM{0.0053}$  & $\colorcellSplaTAM{0.0052}$ & $\colorcellSplaTAM{0.0050}$ & $\colorcellSplaTAM{0.0058}$ & $\colorcellSplaTAM{0.0072}$ & $\colorcellSplaTAM{0.0044}$ & $\colorcellSplaTAM{0.0067}$ & $\colorcellSplaTAM{0.0062}$ & $\colorcellSplaTAM{0.0062}$ & $\colorcellSplaTAM{0.045}$\textit{\textbf{G}} & $\colorcellSplaTAM{0.0041}$ & $\colorcellSplaTAM{0.0054}$ & $\colorcellSplaTAM{0.0096}$ & $\colorcellSplaTAM{0.0046}$ & $\colorcellSplaTAM{0.0045}$  
\\ \midrule
 
        \multicolumn{20}{c}{{Optimal performance (min ATE) achieved by using all SLAM models:}}  \\ \midrule
      min ATE  & \multirow{3}{*}{$\textbf{0.0039}$} & {{{{0.0061}}}}   & {${0.0111}$} & ${0.0107}$ & ${0.0053}$  & ${0.0052}$ & ${0.0050}$ & ${0.0058}$ & ${0.0072}$ & ${0.0044}$ & ${0.0067}$ & ${0.0062}$ & ${0.0062}$ & {${0.0111}$} & ${0.0041}$ & ${0.0051}$ & ${0.0050}$ & ${0.0046}$ & ${0.0044}$  
    \\ \cmidrule{5-8}\cmidrule{9-12}\cmidrule{13-16}\cmidrule{17-20}
     mean(min ATE)& & {{\textbf{\colorcellpurple{0.0061}}}}   & {\colorcellpurple{0.0069}}  &  \multicolumn{4}{c|}{\colorcellpurple{0.0066}}&  \multicolumn{4}{c|}{\colorcellpurple{0.0060}}&  \multicolumn{4}{c|}{\colorcellpurple{0.0069}} &  \multicolumn{4}{c}{\colorcellpurple{\colorcellpurple{0.0048}}}
    \\ 
    \bottomrule  \bottomrule
            \multicolumn{20}{l}{{\textit{{G}} represent settings that include failure sequences where no final trajectory is generated due to running out of GPU memory (more than 48GB).}}\\
            \multicolumn{20}{l}{{{The number in front of \textit{G}} represents the average ATE as failure sequences are set as a value of 1.0.}}\\
    \end{tabular}
}
\end{table*}







==> tables/table_sensor_perturb_performance_bak.tex <==

\begin{table*}[t]
\caption{Performance (ATE RMSE [m]) under image perturbation in the static (top) and dynamic (bottom) perturbation mode. For cases where no final trajectory is produced (e.g., due to tracking loss or out of GPU memory ($>24GB$)), we assign an ATE of 1.0 and calculate the average ATE for each perturbation type. These cases are denoted with an "F" at the end of the result.}
\label{tab:sensor_perturb_static}
\centering\setlength{\tabcolsep}{0.8mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cc|cccc|cccc|cccc|cccc}
    \toprule \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Clean}}&  \multicolumn{2}{|c|}{\textbf{Perturbed}}  & \multicolumn{4}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Environmental Interference}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{5-8} \cmidrule{9-12} \cmidrule{13-16} \cmidrule{17-20}
    &  & \textbf{Mean} & \textbf{Max}  & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{20}{c}{Static Perturbation Mode for Monocular Setting SLAM Models}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{zhang2023goslam} & $0.0039$ & $0.000$  & $0.000$ & $0.0151$ & $0.0052$ & $0.0052$ & $0.0089$ & $0.0776$ & $0.0456$ & $0.0296$ & $0.0190$ & $0.2157$ & $0.7207$ & $0.1921$ & $0.0859$ & $0.0046$ & $0.0047$ & $0.0095$ & $0.0046$ 
   
    \\ \midrule
        \multicolumn{20}{c}{Static Perturbation Mode for RGBD Setting SLAM Models}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{imap} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{niceslam}& $0.0147$ & $0.000$ & $0.000$  & $0.0307$ & $0.0151$ & $0.0161$ & $0.0188$ & $0.0254$ & $0.0377$ & $0.0353$ & $0.0151$ & $0.0186$ & $0.0160$ & $0.0323$ & $0.0320$ & $0.0654$ & $0.0161$ & $0.0150$ & $0.0145$
    \\
    CO-SLAM~\cite{coslam}& $0.0090$ & $0.000$ & $0.000$  & $0.0115$ & $0.0096$ & $0.0097$ & $0.0097$ & $0.0125$ & $0.0101$ & $0.0099$ & $0.0105$ & $0.0118$ & $0.0113$ & $0.0104$ & $0.0098$ & $0.0103$ & $0.0112$ & $0.0094$ & $0.0094$

    \\

    GO-SLAM~\cite{zhang2023goslam} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam-S~\cite{keetha2023splatam}& $0.0045$ & $0.000$ & $0.000$ & $0.0142$ & $0.0054$  & $0.0048$ & $0.0049$ & $0.0056$ & $0.0053$ & $0.0045$ & $0.0049$ & $0.0086$ & $0.0063$ & $0.0049$ & $0.0051$ & $0.0037$ & $0.0121$ & $0.0043$ & $0.0049$  
    \\
    \bottomrule \bottomrule
    \end{tabular}
}
\end{table*}


\begin{table*}[t]
\caption{Performance (ATE RMSE [m]) under image perturbation in the dynamic perturbation mode.}
\label{tab:sensor_perturb_dynamic}
\centering\setlength{\tabcolsep}{0.8mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cc|cccc|cccc|cccc|cccc}
    \toprule \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Clean}}&  \multicolumn{2}{|c|}{\textbf{Perturbed}}  & \multicolumn{4}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Environmental Interference}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{5-8} \cmidrule{9-12} \cmidrule{13-16} \cmidrule{17-20}
    &  & \textbf{Mean} & \textbf{Max}  & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{20}{c}{Dynamic Perturbation Mode for Monocular Setting SLAM Models}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
        GO-SLAM~\cite{zhang2023goslam} & $0.0039$ & $0.000$ & $0.000$ & $0.0155$ & $0.0065$   & $0.0060$ & $0.0090$  & $0.0509$ & $0.0253$ & $0.0396$ & $0.0158$ & $0.2668$ & $0.7395$& $0.2254$  & $0.0474$ & $0.0066$ & $0.0050$ & $0.0298$ & $0.0044$ 
    \\
    \midrule
        \multicolumn{20}{c}{Dynamic Perturbation Mode for RGBD Setting SLAM Models}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{imap} & $0.1209$ & $0.000$ & $0.000$ & $0.1243$ & $0.1042$ & $0.2149$  & $0.1221$ & $0.1354$ & $0.1170$ & $0.1967$ & $0.1576$ & $0.2279$ & $0.2873$ & $0.2412$ & $0.1528$ & $0.2141$ & $0.2576$ & $0.1607$ & $0.0955$ 
    \\
    Nice-SLAM~\cite{niceslam}& $0.0147$ & $0.000$ & $0.000$  & $0.0157$ & $0.0252$ & $0.0359$ & $0.0211$ & $0.0288$ & $0.0409$ & $0.0146$ & $0.0155$ & $0.0167$ & $0.0211$ & $0.0197$ & $0.0187$ & $0.0206$ & $0.0155$ & $0.0146$ & $0.0170$
    \\
    CO-SLAM~\cite{coslam}& $0.0090$ & $0.000$ & $0.000$ & $0.0107$ & $0.0095$ & $0.0115$ & $0.0093$ & $0.0106$ & $0.0103$ & $0.0102$ & $0.0098$ & $0.0117$ & $0.0116$ & $0.0111$ & $0.0109$ & $0.0106$ & $0.0111$ & $0.0095$ & $0.0097$
    \\
 GO-SLAM~\cite{zhang2023goslam} & $0.0046$ & $0.000$  & $0.000$ & $0.0130$ & $0.0057$ & $0.0055$ & $0.0078$ & $0.0185$ & $0.0117$ & $0.0139$ & $0.0098$ & $0.1685$ & $0.2213$ & $0.0637$ & $0.0166$ & $0.0051$ & $0.0052$ & $0.0092$ & $0.0049$ 
    \\ 
    Splatam-S~\cite{keetha2023splatam}& $0.0045$ & $0.000$ & $0.000$ & $0.0195$ & $0.0053$  & $0.0052$ & $0.0050$ & $0.0058$ & $0.0072$ & $0.0043$ & $0.0067$ & $0.0062$ & $0.0063$ & {$0.0469$F} & $0.0040$ & $0.0054$ & $0.0096$ & $0.0045$ & $0.0046$  
    \\
    \bottomrule  \bottomrule
    \end{tabular}
}
\end{table*}





\begin{table*}[t]
\caption{Performance (ATE RMSE [m] ($\downarrow$)) under static (\textbf{Top}) and dynamic (\textbf{Bottom}) image perturbations. }
\label{tab:image_perturb}
\centering\setlength{\tabcolsep}{0.4mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cc|cccc|cccc|cccc|cccc}
    \toprule \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Clean}}&  \multicolumn{2}{|c|}{\textbf{Perturbed}}  & \multicolumn{4}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Environmental Interference}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{5-8} \cmidrule{9-12} \cmidrule{13-16} \cmidrule{17-20}
    &  & \textbf{Mean} & \textbf{Max}  & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{20}{c}{\textbf{Static Perturbation} Mode for \textbf{Monocular} SLAM Models}  \\ \midrule
   %  VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$     \\
    ORBSLAM3~\cite{orbslam3} & $0.0145$ & $0.763F$ & $1.4284$  & $0.891F$ & $0.535F$ & $0.505F$ & $0.797F$ & $0.917F$ & $0.969F$ & $1.000F$ & $0.923F$ & $0.629F$ & $0.917F$ & $1.000F$ & $0.719F$ & ${0.0265}$ & $0.612F$ & $1.000F$ & $0.768F$ 
    \\    
    GO-SLAM~\cite{zhang2023goslam} & $\textbf{0.0039}$ & $\textbf{0.0903}$  & $\textbf{0.7207}$ & $\textbf{0.0151}$ & $\textbf{0.0052}$ & $\textbf{0.0052}$ & $\textbf{0.0089}$ & $\textbf{0.0776}$ & $\textbf{0.0456}$ & $\textbf{0.0296}$ & $\textbf{0.0190}$ & $\textbf{0.2157}$ & $\textbf{0.7207}$ & $\textbf{0.1921}$ & $\textbf{0.0859}$ & $\textbf{0.0046}$ & $\textbf{0.0047}$ & $\textbf{0.0095}$ & $\textbf{0.0046}$ 
   
    \\ \midrule
        \multicolumn{20}{c}{\textbf{Static Perturbation} Mode for \textbf{RGBD} SLAM Models}  \\ \midrule
 %    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$   \\
    ORBSLAM3~\cite{orbslam3} & $0.0823$ & $0.476F$ & $1.1606$ & $0.300F$ & $0.340F$ & $0.292F$ & $0.211F$ & $0.470F$ & $0.433F$ & $0.591F$ & $0.351F$ & $0.397F$ & $0.640F$ & $0.795F$ & $0.508F$ & $0.0649$ & $0.527F$ & $1.00F$ & $0.7034$
    \\
    IMAP~\cite{imap} & $0.1209$ & $0.1568$ & $0.3831$ & $0.1424$ & $0.1671$ & $0.1811$ & $0.0672$ & $0.0278$ & $0.0779$ & $0.1710$ & $0.1087$ & $0.1913$ & $0.1316$ & $0.1665$ & $0.1473$ & $0.1903$ & $0.3831$ & $0.1884$ & $0.1669$  
    \\
    Nice-SLAM~\cite{niceslam}& $0.0147$ & $0.0253$ & $0.0377$  & $0.0307$ & $0.0151$ & $0.0161$ & $0.0188$ & $0.0254$ & $0.0377$ & $0.0353$ & $0.0151$ & $0.0186$ & $0.0160$ & $0.0323$ & $0.0320$ & $0.0654$ & $0.0161$ & $0.0150$ & $0.0145$
    \\
    CO-SLAM~\cite{coslam}& $0.0090$ & $0.0104$ &  $\textbf{0.0125}$  & $\textbf{0.0115}$ & $0.0096$ & $0.0097$ & $0.0097$ & $0.0125$ & $0.0101$ & $0.0099$ & $0.0105$ & $0.0118$ & $0.0113$ & $0.0104$ & $0.0098$ & $0.0103$ & $0.0112$ & $0.0094$ & $0.0094$

    \\

    GO-SLAM~\cite{zhang2023goslam} & $0.0046$ & $0.0574$ &$0.6271$ & $0.0135$ & $\textbf{0.0052}$ & ${0.0052}$ & $0.0090$ & $0.0169$ & $0.0140$ & $0.0171$ & $0.0100$ & $0.1211$ & $0.6271$ & $0.0416$ & $0.0164$ & $0.0047$ & $\textbf{0.0054}$ & $0.0065$ & $0.0050$ 
    \\
    SplaTAM-S~\cite{keetha2023splatam}& $\textbf{0.0045}$ & $\textbf{0.0062}$ & $0.0160$ & $0.0160$ & $\textbf{0.0052}$  & $\textbf{0.0049}$ & $\textbf{0.0048}$ & $\textbf{0.0054}$ & $\textbf{0.0050}$ & $\textbf{0.0044}$ & $\textbf{0.0051}$ & $\textbf{0.0085}$ & $\textbf{0.0063}$ & $\textbf{0.0048}$ & $\textbf{0.0051}$ & $\textbf{0.0038}$ & $0.0133$ & $\textbf{0.0044}$ & $\textbf{0.0048}$  
    \\  \midrule
        \multicolumn{20}{c}{\textbf{\textit{Survival Upper-bound:}} The highest expected performance (min ATE) attainable using all advanced models.}  \\ \midrule
      min ATE  & \multirow{3}{*}{$0.0045$} & \multirow{3}{*}{${0.0056}$}   & {${0.0115}$} & $0.0115$ & $0.0052$  & $0.0049$ & $0.0048$ & $0.0054$ & $0.0050$ & $0.0044$ & $0.0051$ & $0.0085$ & $0.0063$ & $0.0048$ & $0.0051$ & $0.0038$ & $0.0054$ & $0.0044$ & $0.0048$  
    \\ \cmidrule{5-8}\cmidrule{9-12}\cmidrule{13-16}\cmidrule{17-20}
     mean(min ATE)& &  & {0.0066}  &  \multicolumn{4}{c|}{${0.0066}$}&  \multicolumn{4}{c|}{$0.0050$}&  \multicolumn{4}{c|}{$0.0062$} &  \multicolumn{4}{c}{$0.0046$}
    \\ 
       \midrule     \midrule
    \multicolumn{20}{c}{\textbf{Dynamic Perturbation} Mode for \textbf{Monocular} SLAM Models}  \\ \midrule
  %   VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$   \\
    ORBSLAM3~\cite{orbslam3} & $0.0145$ & $0.854F$ & $1.2481$  & $0.925F$ & $0.506F$ & $0.760F$ & $0.813F$ & $1.000F$ & $1.000F$ & $1.000F$ & $0.885F$ & $0.751F$ & $1.000F$ & $1.000F$ & $1.000F$ & $0.0517$ & $1.000F$ & $1.000F$ & $0.718F$ 
    \\    
        GO-SLAM~\cite{zhang2023goslam} & $\textbf{0.0039}$ & $\textbf{0.0933}$ & $\textbf{0.7395}$ & $\textbf{0.0155}$ & $\textbf{0.0065}$   & $\textbf{0.0060}$ & $\textbf{0.0090}$  & $\textbf{0.0509}$ & $\textbf{0.0253}$ & $\textbf{0.0396}$ & $\textbf{0.0158}$ & $\textbf{0.2668}$ & $\textbf{0.7395}$& $\textbf{0.2254}$  & $\textbf{0.0474}$ & $\textbf{0.0066}$ & $\textbf{0.0050}$ & $\textbf{0.0298}$ & $\textbf{0.0044}$ 
    \\
    \midrule
        \multicolumn{20}{c}{\textbf{Dynamic Perturbation} Mode for \textbf{RGBD} SLAM Models}  \\ \midrule
  %   VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$     \\
   ORBSLAM3~\cite{orbslam3} & $0.0823$ & $0.594F$ & $1.0629$  & $0.279F$ & $0.303F$ & $0.0515$ & $0.1680$ & $0.508F$ & $0.513F$ & $0.755F$ & $0.262F$ & $0.659F$ & $0.256F$ & $0.876F$ & $0.753F$ & $0.0660$ & $0.751F$ & $1.000F$ & $0.756F$ 
    \\
    IMAP~\cite{imap} & $0.1209$ & $0.1756$ & $0.2873$ & $0.1243$ & $0.1042$ & $0.2149$  & $0.1221$ & $0.1354$ & $0.1170$ & $0.1967$ & $0.1576$ & $0.2279$ & $0.2873$ & $0.2412$ & $0.1528$ & $0.2141$ & $0.2576$ & $0.1607$ & $0.0955$ 
    \\
    Nice-SLAM~\cite{niceslam}& $0.0147$ & $0.0214$ &$0.0409$ & $0.0157$ & $0.0252$ & $0.0359$ & $0.0211$ & $0.0288$ & $0.0409$ & $0.0146$ & $0.0155$ & $0.0167$ & $0.0211$ & $0.0197$ & $0.0187$ & $0.0206$ & $0.0155$ & $0.0146$ & $0.0170$
    \\
    CO-SLAM~\cite{coslam}& $0.0090$ & $0.0105$ & $\textbf{0.0117}$ & $\textbf{0.0107}$ & $0.0095$ & $0.0115$ & $0.0093$ & $0.0106$ & $0.0103$ & $0.0102$ & $0.0098$ & $0.0117$ & $0.0116$ & $\textbf{0.0111}$ & $0.0109$ & $0.0106$ & $0.0111$ & $0.0095$ & $0.0097$
    \\
 GO-SLAM~\cite{zhang2023goslam} & $0.0046$ & $0.0363$  & $0.2213$ & $0.0130$ & $0.0057$ & $0.0055$ & $0.0078$ & $0.0185$ & $0.0117$ & $0.0139$ & $0.0098$ & $0.1685$ & $0.2213$ & $0.0637$ & $0.0166$ & $\textbf{0.0051}$ & $\textbf{0.0052}$ & $0.0092$ & $0.0049$ 
    \\ 
    SplaTAM-S~\cite{keetha2023splatam}& $\textbf{0.0045}$ & $\textbf{0.008}F$ & {$0.045$F} & $0.0191$ & $\textbf{0.0053}$  & $\textbf{0.0052}$ & $\textbf{0.0050}$ & $\textbf{0.0058}$ & $\textbf{0.0072}$ & $\textbf{0.0044}$ & $\textbf{0.0067}$ & $\textbf{0.0062}$ & $\textbf{0.0062}$ & {$0.045$F} & $\textbf{0.0041}$ & $0.0054$ & $0.0096$ & $\textbf{0.0046}$ & $\textbf{0.0045}$  
    \\     \midrule
        \multicolumn{20}{c}{\textbf{\textit{Survival Upper-bound:}} The highest expected performance (min ATE) attainable using all advanced models.}  \\ \midrule
      min ATE  & \multirow{3}{*}{$0.0045$} & \multirow{3}{*}{${0.0061}$}   & {${0.0111}$} & ${0.0107}$ & ${0.0053}$  & ${0.0052}$ & ${0.0050}$ & ${0.0058}$ & ${0.0072}$ & ${0.0044}$ & ${0.0067}$ & ${0.0062}$ & ${0.0062}$ & {${0.0111}$} & ${0.0041}$ & ${0.0051}$ & ${0.0052}$ & ${0.0046}$ & ${0.0045}$  
    \\ \cmidrule{5-8}\cmidrule{9-12}\cmidrule{13-16}\cmidrule{17-20}
     mean(min ATE)& &  & {${0.0069}$}  &  \multicolumn{4}{c|}{0.0066}&  \multicolumn{4}{c|}{0.0060}&  \multicolumn{4}{c|}{0.0069} &  \multicolumn{4}{c}{0.0049}
    \\ 
    \bottomrule  \bottomrule
     \multicolumn{20}{l}{{\textbf{1}) We highlight the best performance, \textit{i.e.}, the lowest ATE, under each perturbation type for static and dynamic perturbation mode in \textbf{bold}. }}\\
    \multicolumn{20}{l}{{\textbf{2}) Notation $\textbf{F}$ is to denote cases where no final trajectory is generated, which may occur due to tracking loss at the initial stage or insufficient GPU memory. It is important to note  }}\\
        \multicolumn{20}{l}{{that when calculating the ATE metric for such instances, we assign a value of 1.0 for further per-setting average.}}\\
        \multicolumn{20}{l}{{\textbf{3}) As neural models can estimate the entire trajectory, we calculate ATE on the complete trajectory. Notice that a high ATE (\textit{e.g.}, $\geq$ 0.2 [m])  is typically correlated to tracking loss.}}\\
        \multicolumn{20}{l}{{However, as ORBSLAM3~\cite{orbslam3} stops to predict subsequent frames when losing track, we follow previous literature~\cite{wang2020tartanair} to present ATE calculated with tracked partial trajectory.}}\\
            \multicolumn{20}{l}{{Hence, please be aware that a direct quantitative comparison between the ATE results of classical and neural SLAM models should be handled with caution.}}\\
    \end{tabular}
}
\end{table*}


==> tables/table_traj_perturb_performance_cs_metric_10cm.tex <==



\begin{table*}[t]
    \centering
    \begin{minipage}[t!]{0.70\textwidth}
   % \vspace{-10mm}
       \caption{Performance (Categorical Success Rate, CSR($\delta_2$) ($\uparrow$), with 10cm error tolerance, \textit{i.e.}, $\delta_2=10cm$) under trajectory-level perturbation.}
\centering\setlength{\tabcolsep}{0.6mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccc|cccc|cccc|cccc}
    \toprule \toprule
     \textbf{Rotate [$\deg$]} & \multirow{2}{*}{\textbf{Clean}}  & \multicolumn{3}{c|}{\textbf{\textit{0}}} & \multicolumn{4}{c|}{\textbf{\textit{1}}} & \multicolumn{4}{c|}{\textbf{\textit{3}}} & \multicolumn{4}{c}{\textbf{\textit{5}}}
    \\ \cmidrule{1-1} \cmidrule{3-5} \cmidrule{6-9} \cmidrule{10-13} \cmidrule{14-17}
     \textbf{Translate  [$m$]} &  & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} & \textit{\textbf{0}} & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} & \textit{\textbf{0}}  & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} & \textit{\textbf{0}} & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} 
    \\\midrule\midrule
    \multicolumn{17}{c}{Monocular Setting}  \\ \midrule
    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    GO-SLAM~\cite{zhang2023goslam} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  
    \\ \midrule
        \multicolumn{17}{c}{RGBD Setting}  \\ \midrule
    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$
    \\
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{imap} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{niceslam}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{coslam}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
%    rot_0_tran_0           0.016603
%rot_0_tran_0dot0125    0.041986
%rot_0_tran_0dot025     0.084848
%rot_0_tran_0dot05      0.308709
%rot_1_tran_0           0.457948
%rot_1_tran_0dot0125    0.506852
%rot_1_tran_0dot025     0.299822
%rot_1_tran_0dot05      0.504097
%rot_3_tran_0           0.644292
%rot_3_tran_0dot0125    0.662984
%rot_3_tran_0dot025     0.753216
%rot_3_tran_0dot05      0.577154
%rot_5_tran_0           0.845708
%rot_5_tran_0dot0125    0.796604
%rot_5_tran_0dot025     0.827732
%rot_5_tran_0dot05      1.004492

    GO-SLAM~\cite{zhang2023goslam} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
Splatam-S~\cite{keetha2023splatam}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule \bottomrule
    \end{tabular}
}
         \label{tab:trajectory-perturbation}
    \end{minipage}
    \hfill 
    \begin{minipage}[t!]{0.295\textwidth}
    \caption{Performance ( CSR($\delta_2$) ($\uparrow$) under fatser motion.}%\vspace{-3mm}
\label{tab:faster_motion_benchmark}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccc}
    \toprule \toprule
     {\textbf{Method}}
     & \textbf{$1\times$} & \textbf{$2\times$} & \textbf{$4\times$} & \textbf{$8\times$}    \\ \midrule
    \multicolumn{5}{c}{Monocular Setting}  \\ \midrule
    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$  
    \\
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$  
    \\    
    GO-SLAM${}^{\dagger}$~\cite{zhang2023goslam} & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{zhang2023goslam} & $100.0$ & $\textbf{100.0}$ & $\textbf{100.0}$ & $\textbf{100.0}$ 
    \\ \midrule
        \multicolumn{5}{c}{RGBD Setting}  \\ \midrule
    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$  
    \\
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{imap}& $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{niceslam} & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{coslam}& $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    GO-SLAM${}^{\dagger}$~\cite{zhang2023goslam} & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{zhang2023goslam} & $100.0$ & $100.0$ & $100.0$ & $100.0$ 
    \\
Splatam-S~\cite{keetha2023splatam}& $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    % 0.004430484243236739
    \\
    \bottomrule \bottomrule
    \multicolumn{5}{l}{{$\dagger$ denotes  loop closure mechanism is disabled.}}\\
    \end{tabular}
}
        \label{tab:faster-motion-perturbation}
    \end{minipage}
\end{table*}




==> tables/table_traj_perturb_performance_cs_metric_20cm.tex <==



\begin{table*}[t]
    \centering
    \begin{minipage}[t!]{0.70\textwidth}
   % \vspace{-10mm}
       \caption{Performance (Categorical Success Rate, CSR($\delta_3$) ($\uparrow$), with 20cm error tolerance, \textit{i.e.}, $\delta_3=20cm$) under trajectory-level perturbation.}
\centering\setlength{\tabcolsep}{0.6mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccc|cccc|cccc|cccc}
    \toprule \toprule
     \textbf{Rotate [$\deg$]} & \multirow{2}{*}{\textbf{Clean}}  & \multicolumn{3}{c|}{\textbf{\textit{0}}} & \multicolumn{4}{c|}{\textbf{\textit{1}}} & \multicolumn{4}{c|}{\textbf{\textit{3}}} & \multicolumn{4}{c}{\textbf{\textit{5}}}
    \\ \cmidrule{1-1} \cmidrule{3-5} \cmidrule{6-9} \cmidrule{10-13} \cmidrule{14-17}
     \textbf{Translate  [$m$]} &  & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} & \textit{\textbf{0}} & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} & \textit{\textbf{0}}  & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} & \textit{\textbf{0}} & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} 
    \\\midrule\midrule
    \multicolumn{17}{c}{Monocular Setting}  \\ \midrule
    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    GO-SLAM~\cite{zhang2023goslam} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  
    \\ \midrule
        \multicolumn{17}{c}{RGBD Setting}  \\ \midrule
    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$
    \\
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{imap} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{niceslam}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{coslam}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
%    rot_0_tran_0           0.016603
%rot_0_tran_0dot0125    0.041986
%rot_0_tran_0dot025     0.084848
%rot_0_tran_0dot05      0.308709
%rot_1_tran_0           0.457948
%rot_1_tran_0dot0125    0.506852
%rot_1_tran_0dot025     0.299822
%rot_1_tran_0dot05      0.504097
%rot_3_tran_0           0.644292
%rot_3_tran_0dot0125    0.662984
%rot_3_tran_0dot025     0.753216
%rot_3_tran_0dot05      0.577154
%rot_5_tran_0           0.845708
%rot_5_tran_0dot0125    0.796604
%rot_5_tran_0dot025     0.827732
%rot_5_tran_0dot05      1.004492

    GO-SLAM~\cite{zhang2023goslam} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
Splatam-S~\cite{keetha2023splatam}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule \bottomrule
    \end{tabular}
}
         \label{tab:trajectory-perturbation}
    \end{minipage}
    \hfill 
    \begin{minipage}[t!]{0.295\textwidth}
    \caption{Performance ( CSR($\delta_3$) ($\uparrow$) under fatser motion.}%\vspace{-3mm}
\label{tab:faster_motion_benchmark}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccc}
    \toprule \toprule
     {\textbf{Method}}
     & \textbf{$1\times$} & \textbf{$2\times$} & \textbf{$4\times$} & \textbf{$8\times$}    \\ \midrule
    \multicolumn{5}{c}{Monocular Setting}  \\ \midrule
    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$  
    \\
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$  
    \\    
    GO-SLAM${}^{\dagger}$~\cite{zhang2023goslam} & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{zhang2023goslam} & $100.0$ & $100.0$ & $100.0$ & $100.0$ 
    \\ \midrule
        \multicolumn{5}{c}{RGBD Setting}  \\ \midrule
    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$  
    \\
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{imap}& $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{niceslam} & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{coslam}& $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    GO-SLAM${}^{\dagger}$~\cite{zhang2023goslam} & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{zhang2023goslam} & $100.0$ & $100.0$ & $100.0$ & $100.0$ 
    \\
Splatam-S~\cite{keetha2023splatam}& $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    % 0.004430484243236739
    \\
    \bottomrule \bottomrule
    \multicolumn{5}{l}{{$\dagger$ denotes  loop closure mechanism is disabled.}}\\
    \end{tabular}
}
        \label{tab:faster-motion-perturbation}
    \end{minipage}
\end{table*}




==> tables/table_traj_perturb_performance_cs_metric_5cm.tex <==



\begin{table*}[t]
    \centering
    \begin{minipage}[t!]{0.70\textwidth}
   % \vspace{-10mm}
       \caption{Performance (Categorical Success Rate, CSR($\delta_1$) ($\uparrow$), with 5cm error tolerance, \textit{i.e.}, $\delta_1=5cm$) under trajectory-level perturbation.}
\centering\setlength{\tabcolsep}{0.6mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccc|cccc|cccc|cccc}
    \toprule \toprule
     \textbf{Rotate [$\deg$]} & \multirow{2}{*}{\textbf{Clean}}  & \multicolumn{3}{c|}{\textbf{\textit{0}}} & \multicolumn{4}{c|}{\textbf{\textit{1}}} & \multicolumn{4}{c|}{\textbf{\textit{3}}} & \multicolumn{4}{c}{\textbf{\textit{5}}}
    \\ \cmidrule{1-1} \cmidrule{3-5} \cmidrule{6-9} \cmidrule{10-13} \cmidrule{14-17}
     \textbf{Translate  [$m$]} &  & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} & \textit{\textbf{0}} & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} & \textit{\textbf{0}}  & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} & \textit{\textbf{0}} & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} 
    \\\midrule\midrule
    \multicolumn{17}{c}{Monocular Setting}  \\ \midrule
    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    GO-SLAM~\cite{zhang2023goslam} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  
    \\ \midrule
        \multicolumn{17}{c}{RGBD Setting}  \\ \midrule
    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$
    \\
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{imap} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{niceslam}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{coslam}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
%    rot_0_tran_0           0.016603
%rot_0_tran_0dot0125    0.041986
%rot_0_tran_0dot025     0.084848
%rot_0_tran_0dot05      0.308709
%rot_1_tran_0           0.457948
%rot_1_tran_0dot0125    0.506852
%rot_1_tran_0dot025     0.299822
%rot_1_tran_0dot05      0.504097
%rot_3_tran_0           0.644292
%rot_3_tran_0dot0125    0.662984
%rot_3_tran_0dot025     0.753216
%rot_3_tran_0dot05      0.577154
%rot_5_tran_0           0.845708
%rot_5_tran_0dot0125    0.796604
%rot_5_tran_0dot025     0.827732
%rot_5_tran_0dot05      1.004492

    GO-SLAM~\cite{zhang2023goslam} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
Splatam-S~\cite{keetha2023splatam}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule \bottomrule
    \end{tabular}
}
         \label{tab:trajectory-perturbation}
    \end{minipage}
    \hfill 
    \begin{minipage}[t!]{0.295\textwidth}
    \caption{Performance ( CSR($\delta_1$) ($\uparrow$) under fatser motion.}%\vspace{-3mm}
\label{tab:faster_motion_benchmark}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccc}
    \toprule \toprule
     {\textbf{Method}}
     & \textbf{$1\times$} & \textbf{$2\times$} & \textbf{$4\times$} & \textbf{$8\times$}    \\ \midrule
    \multicolumn{5}{c}{Monocular Setting}  \\ \midrule
    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$  
    \\
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$  
    \\    
    GO-SLAM${}^{\dagger}$~\cite{zhang2023goslam} & $0.000$ & $0.000$ & $0.000$ & $0.000$  
    \\
    GO-SLAM~\cite{zhang2023goslam} & $0.000$  & $87.5$ & $62.5$ & $62.5$ 
    \\ \midrule
        \multicolumn{5}{c}{RGBD Setting}  \\ \midrule
    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$  
    \\
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{imap}& $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{niceslam} & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{coslam}& $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    GO-SLAM${}^{\dagger}$~\cite{zhang2023goslam}& $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{zhang2023goslam}  & $0.000$ & $75.0$ & $62.5$ & $50.0$ 
    \\
Splatam-S~\cite{keetha2023splatam}& $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    % 0.004430484243236739
    \\
    \bottomrule \bottomrule
    \multicolumn{5}{l}{{$\dagger$ denotes  loop closure mechanism is disabled.}}\\
    \end{tabular}
}
        \label{tab:faster-motion-perturbation}
    \end{minipage}
\end{table*}



